ResKD: Residual-Guided Knowledge Distillation

Knowledge distillation, aimed at transferring the knowledge from a heavy teacher network to a lightweight student network, has emerged as a promising technique for compressing neural networks. However, due to the capacity gap between the heavy teacher and the lightweight student, there still exists a significant performance gap between them. In this paper, we see knowledge distillation in a fresh light, using the knowledge gap, or the residual, between a teacher and a student as guidance to train a much more lightweight student, called a res-student. We combine the student and the res-student into a new student, where the res-student rectifies the errors of the former student. Such a residual-guided process can be repeated until the user strikes the balance between accuracy and cost. At inference time, we propose a sample-adaptive strategy to decide which res-students are not necessary for each sample, which can save computational cost. Experimental results show that we achieve competitive performance with 18.04$\%$, 23.14$\%$, 53.59$\%$, and 56.86$\%$ of the teachers' computational costs on the CIFAR-10, CIFAR-100, Tiny-ImageNet, and ImageNet datasets. Finally, we do thorough theoretical and empirical analysis for our method.

==> minor_sup/KD_method.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{The results of different distillation methods on CIFAR-100. $T$ is ResNet-110, $S_0$ is ResNet-20, $S_{big}$ is ResNet-32, and $S_1$ (ResNet20) is a NAS-based network combined with $S_0$, ResNet-20.
        We report ``$S_1$ Accuracy (Gap to $S_0$) (Gap to $S_{big}$)'' as ``75.75 (+4.14 / +4.19) (+1.35 / +2.00)''. 
        75.75 is accuracy of $S_1$, ``(+4.14 / +4.19)'' means $S_1$ accuracy have a +4.14 / +4.19 gap compared with its $S_0$, and ``(+1.35 / +2.00)'' means $S_1$ accuracy have a +1.35 / +2.00 gap compared with corresponding $S_{big}$.
        We report ``$S_1$ MFlops (Gap to $S_0$) (Gap to $S_{big}$)'' as ``57.37 (+16.15) (-12.39)''. 
        57.37 is the MFlops of  $S_1$, +16.15 means $S_1$ has 16.15M more Flops than its $S_0$, and -12.39 means $S_1$ has 12.39M fewer Flops than corresponding $S_{big}$.
        % ``KD'' means the original knowledge distillation method [15].
        For a fair comparison, we control the cost of all $S_1$ with a similar level.
        Our ResKD can work well with different distillation methods.
        }
        \label{table.KD_method}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \begin{tabular}{ccccl}
            \toprule
        

        KD& $T$ Accuracy (\%) & $S_0$ Accuracy (\%)&$S_{big}$ Accuracy (\%)  &$S_1$ Accuracy (Gap to $S_0$) (Gap to $S_{big}$) (\%)  \\
        Method& $T$ MFlops & $S_0$ MFlops&$S_{big}$ MFlops &$S_1$ MFlops (Gap to $S_0$) (Gap to $S_{big}$)\\
        \toprule
        % \multicolumn{5}{l}{\emph{Prediction Distillation}} \\
        
        % \multirow{2}{*}{KD}&74.31&71.03 / 70.67 [r2]&74.03 / 73.08 [r2]& 75.69 (+4.66 / +5.02) (+1.66 / +2.61) \\
        % &255.28& 41.22 &69.76& 56.96 (+15.74) (-12.80)  \\
        % \toprule
        \multicolumn{5}{l}{\emph{Feature Distillation}} \\
        \multirow{2}{*}{FitNet}&74.31&69.65 / 68.99 [r2]&70.92 / 71.06 [r2] & 75.12 (+5.47 / +6.13) (+4.20 / +4.06)	 \\
        &255.28& 41.22 &69.76& 64.49 (+23.27) (-5.27)\\
        \toprule
        \multirow{2}{*}{CRD}&74.31&71.33 / 71.46 [r2]& 73.87 / 73.48
        [r2]
        & 76.07 (+4.74 / +4.61) (+2.20 / +2.59) \\
        &255.28& 41.22 &69.76& 62.80 (+21.58) (-6.96)   \\
        \toprule
        \multicolumn{5}{l}{\emph{Both Prediction and Feature Distillation}} \\
        \multirow{2}{*}{CRD+KD}&74.31&71.61 /  71.56 [r2]&74.40	/ 73.75 [r2]
        & 75.75 (+4.14 / +4.19) (+1.35 / +2.00)  \\
        &255.28& 41.22 &69.76& 57.37 (+16.15) (-12.39)   \\
        
        \bottomrule%
        
        \end{tabular}
        
        \end{center}
        \end{table*}



==> minor_sup/KD_method20.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{The results of different distillation methods on CIFAR-100. $T$ is ResNet-110, $S_0$ is ResNet-20, and $S_1$ is a NAS-based network combined with $S_0$, ResNet-20.
        We report the accuracy gap as +4.14 / +4.19 [33], which means $S_1$ has 4.14 / 4.19 \% better accuracy than $S_0$ based on our reimplementation / the accuracy reported by [33].
        % ``KD'' means the original knowledge distillation method [15].
        For a fair comparison, we control the cost of all $S_1$ with a similar level.
        Our ResKD can work well with different distillation methods.
        }
        \label{table.KD_method20}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \begin{tabular}{ccccc}
            \toprule
        

        KD& $T$ Accuracy (\%) & $S_0$ Accuracy (\%)&$S_1$ Accuracy (\%)&Accuracy Gap (\%)  \\
        Method& $T$ MFLOPs & $S_0$ MFLOPs &$S_1$ MFLOPps &MFLOPs Gap\\
        \toprule
        % \multicolumn{5}{l}{\emph{Prediction Distillation}} \\
        
        % \multirow{2}{*}{KD}&74.31&71.03 / 70.67 [r2]&74.03 / 73.08 [r2]& 75.69 (+4.66 / +5.02) (+1.66 / +2.61) \\
        % &255.28& 41.22 &69.76& 56.96 (+15.74) (-12.80)  \\
        % \toprule
        \multicolumn{5}{l}{\emph{Feature Distillation}} \\
        \multirow{2}{*}{FitNet [21]}&74.31&69.65 / 68.99 [33]& 75.12 &+5.47 / +6.13 \\
        &255.28& 41.22 & 64.49 &+23.27\\
        \midrule
        \multirow{2}{*}{AT [23]}&74.31& 70.5 / 70.22 [33] & 75.65& +5.15 / +5.43\\
        &255.28& 41.22& 63.74& +22.52 \\
        \midrule
        \multirow{2}{*}{SP [24]}&74.31& 70.72 / 70.04 [33] & 75.44&+4.72 / +5.40\\
        &255.28& 41.22& 63.63& +22.41  \\
        \midrule
        \multirow{2}{*}{CC [59]}&74.31&69.44 / 69.48 [33] &75.34 &+5.90 / +5.86
        \\
        &255.28& 41.22 & 65.72 & +24.50  \\
        \midrule
        \multirow{2}{*}{VID [28]}&74.31&70.22 / 70.16 [33] & 76.10&+5.88 / +5.94 \\
        &255.28& 41.22& 63.46& +22.24  \\
        \midrule
        \multirow{2}{*}{RKD [26]}&74.31& 69.40 / 69.25 [33] &75.52&+6.12 / +6.27
        \\
        &255.28& 41.22 & 64.97 & +23.75  \\
        \midrule
        \multirow{2}{*}{PKT [30]}&74.31& 70.38 / 70.25 [33] & 75.82&+5.44 / +5.57\\
        &255.28& 41.22& 64.02& +22.80 \\
        \midrule
        \multirow{2}{*}{AB [32]}&74.31& 69.94 / 69.53 [33] & 77.11&+7.17 / 7.58\\
        &255.28& 41.22& 64.75& +22.53 \\
        \midrule
        \multirow{2}{*}{FT [31]}&74.31& 70.06 / 70.22 [33] & 75.78&+5.72 / +5.56\\
        &255.28&  41.22& 64.45& +22.53 \\
        \midrule
        \multirow{2}{*}{NST [29]}&74.31& 70.24 / 69.53 [33] & 75.93&+5.69 / +6.40\\
        &255.28& 41.22& 64.45& +22.53  \\
        \midrule
        \multirow{2}{*}{CRD [33]}&74.31&71.33 / 71.46 [33] & 76.07 &+4.74 / +4.61\\
        &255.28& 41.22 & 62.80& +21.58  \\
        \midrule
        \multicolumn{5}{l}{\emph{Both Prediction and Feature Distillation}} \\
        \multirow{2}{*}{CRD+KD [33]}&74.31&71.61 /  71.56 [33] & 75.75 &+4.14 / +4.19 \\
        &255.28& 41.22 & 57.37 &+16.15  \\
        
        \bottomrule%
        
        \end{tabular}
        
        \end{center}
        \end{table*}


==> minor_sup/KD_method20new.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{ The results of different distillation methods on CIFAR-100. $T$ is ResNet-110 with an accuracy of 74.31\% and a cost of 255.28 MFLOPs. $S_0$ is ResNet-20. $S_1$ is a NAS-based network $R_1$ combined with $S_0$.
        We report the accuracy as ``69.65 / 68.99 [33]'', which means that the re-implemented accuracy is 69.65, and the reported accuracy in [33] is 68.99.
        %We report the accuracy gap as +4.14 / +4.19 [33], which means $S_1$ has 4.14 / 4.19 \% better accuracy than $S_0$ based on our reimplementation / the accuracy reported by [33].
        % ``KD'' means the original knowledge distillation method [15].
        For a fair comparison, we control the cost of all $S_1$ at a similar level.
        Our ResKD can work well with different distillation methods.
        }
        \label{table.KD_method20}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
            %\footnotesize
        \begin{tabular}{llll}
            \toprule

        KD Method & Model &Accuracy (\%)&MFLOPs \\
        %\toprule
        %\multicolumn{4}{l}{\emph{Teacher}} \\
        %&Res110&74.31&255.28\\
        \toprule
        \multicolumn{4}{l}{\emph{Feature Distillation}} \\
        
        \multirow{2}{*}{FitNet [21]} & $S_0$ &69.65 / 68.99 [33]&41.22\\
                                     & $S_1$ &75.12 (\textcolor{red}{$+$5.47 / $+$6.13})&64.49 (\textcolor{red}{$+$23.27})\\
        \midrule
        \multirow{2}{*}{AT [23]}     & $S_0$ & 70.50 / 70.22 [33] &41.22\\
                                     & $S_1$ &75.65 (\textcolor{red}{$+$5.15 / $+$5.43})&63.74 (\textcolor{red}{$+$22.52})\\
        \midrule
        \multirow{2}{*}{SP [24]}     & $S_0$ & 70.72 / 70.04 [33] &41.22\\
                                     & $S_1$ &75.44 (\textcolor{red}{$+$4.72 / $+$5.40})&63.63 (\textcolor{red}{$+$22.41})\\
        \midrule
        \multirow{2}{*}{CC [59]}     & $S_0$ & 69.44 / 69.48 [33] &41.22\\
                                     & $S_1$ &75.34  (\textcolor{red}{$+$5.90 / $+$5.86})&65.72 (\textcolor{red}{$+$24.50})\\
        \midrule
        \multirow{2}{*}{VID [28]}    & $S_0$ & 70.22 / 70.16 [33] &41.22\\
                                     & $S_1$ & 76.10 (\textcolor{red}{$+$5.88 / $+$5.94})  &63.46 (\textcolor{red}{$+$22.24}) \\
        \midrule
        \multirow{2}{*}{RKD [26]}    & $S_0$ & 69.40 / 69.25 [33] &41.22\\
                                     & $S_1$ &75.52 (\textcolor{red}{$+$6.12 / $+$6.27})&64.97 (\textcolor{red}{$+$23.75})\\
        \midrule
        \multirow{2}{*}{PKT [30]}    & $S_0$ & 70.38 / 70.25 [33] &41.22\\
                                     & $S_1$ &75.82 (\textcolor{red}{$+$5.44 / $+$5.57})&64.02 (\textcolor{red}{$+$22.80})\\
        \midrule
        \multirow{2}{*}{AB [32]}     & $S_0$ & 69.94 / 69.53 [33] &41.22\\
                                     & $S_1$ &77.11 (\textcolor{red}{$+$7.17 / $+$7.58})& 64.75 (\textcolor{red}{$+$23.53})\\
        \midrule
        \multirow{2}{*}{FT [31]}     & $S_0$ &  70.06 / 70.22 [33] &41.22\\
                                     & $S_1$ &75.78 (\textcolor{red}{$+$5.72 / $+$5.56})& 64.45 (\textcolor{red}{$+$23.23})\\
        \midrule
        \multirow{2}{*}{NST [29]}    & $S_0$ &  70.24 / 69.53 [33] &41.22\\
                                     & $S_1$ &75.93 (\textcolor{red}{$+$5.69 / $+$6.40})& 64.46 (\textcolor{red}{$+$23.24})\\
        \midrule
        \multirow{2}{*}{CRD [33]}    & $S_0$ &  71.33 / 71.46 [33] &41.22\\
                                     & $S_1$ &76.07  (\textcolor{red}{$+$4.74 / $+$4.61})& 62.80 (\textcolor{red}{$+$21.58})\\
        \toprule
        \multicolumn{4}{l}{\emph{Both Prediction and Feature Distillation}}\\
        \multirow{2}{*}{CRD+KD [33]} & $S_0$ &71.61 /  71.56 [33] &41.22\\
                                     & $S_1$ & 75.75  (\textcolor{red}{$+$4.14 / $+$4.19})& 57.37 (\textcolor{red}{$+$16.15})\\
        \bottomrule%
        
        \end{tabular}
        
        \end{center}
        \end{table*}


==> minor_sup/KD_method32.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{The results of different distillation methods on CIFAR-100. $T$ and $S_1$ is the same ones in \cref{table.KD_method20}.
        $S_{big}$ is ResNet-32.
        We report the accuracy gap as +1.35 / +2.00, which means $S_1$ has 1.35 / 2.00 \% better accuracy than $S_{big}$ based on our reimplementation / the accuracy reported by [r2].
        % ``KD'' means the original knowledge distillation method [15].
        For a fair comparison, we control the cost of all $S_1$ with a similar level.
        Our ResKD can work well with different distillation methods.
        }
        \label{table.KD_method32}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \begin{tabular}{ccccc}
            \toprule
        

        KD& $T$ Accuracy (\%)&$S_{big}$ Accuracy (\%)  &$S_1$ Accuracy  (\%)&Accuracy Gap (\%)  \\
        Method& $T$ MFlops &$S_{big}$ MFlops &$S_1$ MFlops &MFlops Gap \\
        \toprule
        % \multicolumn{5}{l}{\emph{Prediction Distillation}} \\
        
        % \multirow{2}{*}{KD}&74.31&71.03 / 70.67 [r2]&74.03 / 73.08 [r2]& 75.69 (+4.66 / +5.02) (+1.66 / +2.61) \\
        % &255.28& 41.22 &69.76& 56.96 (+15.74) (-12.80)  \\
        % \toprule
        \multicolumn{5}{l}{\emph{Feature Distillation}} \\
        \multirow{2}{*}{FitNet [21]}&74.31&70.92 / 71.06 [33] & 75.12 &+4.20 / +4.06 \\
        &255.28& 69.76& 64.49& -5.27\\
        \midrule
        \multirow{2}{*}{AT [23]}&74.31& 72.80 / 72.31 [33] & 75.65& +2.85 / +3.34        \\
        &255.28& 69.76& 63.74& -6.02  \\
        \midrule
        \multirow{2}{*}{SP [24]}&74.31& 72.81 / 72.69 [33] & 75.44&+2.63 / +2.75        \\
        &255.28& 69.76& 63.63& -6.13  \\
        \midrule
        \multirow{2}{*}{CC [59]}&74.31& 71.89 / 71.48 [33] & 75.34&+3.45 / +3.86\\
        &255.28& 69.76& 65.72& -4.04  \\
        \midrule
        \multirow{2}{*}{VID [28]}&74.31&72.60 / 72.61 [33] & 76.10&+3.5 / +3.49\\
        &255.28& 69.76& 63.46& -6.30  \\
        \midrule
        \multirow{2}{*}{RKD [26]}&74.31& 72.51 / 71.82 [33] & 75.52&+3.01 / +3.70\\
        &255.28& 69.76& 64.97& -4.79  \\
        \midrule
        \multirow{2}{*}{PKT [30]}&74.31& 73.38 / 72.61 [33] & 75.82&+2.44 / +3.21\\
        &255.28& 69.76& 64.02& -5.74  \\
        \midrule
        \multirow{2}{*}{AB [32]}&74.31& 71.73 / 70.98 [33] & 77.11&+5.38 / +6.13\\
        &255.28& 69.76& 64.75& -5.01  \\
        \midrule
        \multirow{2}{*}{FT [31]}&74.31& 72.68 / 72.37 [33] & 75.78&+3.10 / +3.41\\
        &255.28& 69.76& 64.45& -5.31  \\
        \midrule
        \multirow{2}{*}{NST [29]}&74.31& 72.37 / 71.96 [33] & 75.93&+3.56 / +3.97\\
        &255.28& 69.76& 64.45& -5.31  \\
        \midrule
        \multirow{2}{*}{CRD [33]}&74.31& 73.87 / 73.48 [33] & 76.07&+2.20 / +2.59\\
        &255.28& 69.76& 62.80& -6.96  \\
        \midrule
        \multicolumn{5}{l}{\emph{Both Prediction and Feature Distillation}} \\
        \multirow{2}{*}{CRD+KD [33]}&74.31&74.40	/ 73.75 [33]& 75.75 &+1.35 / +2.00 \\
        &255.28 &69.76& 57.37& -12.39 \\
       



        \bottomrule%
        
        \end{tabular}
        
        \end{center}
        \end{table*}

==> minor_sup/KD_method32new.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{
        The results of different distillation methods on CIFAR-100. 
        $T$ is ResNet-110 with an accuracy of 74.31\% and a cost of 255.28 MFLOPs. $S_0$ is ResNet-20. $S_1$ is a NAS-based network $R_1$ combined with $S_0$.
        We compare our $S_1$ with ResNet-32.
        We report the accuracies as ``70.92 / 71.06 [33]'', which means that the re-implemented accuracy is 70.92 and the reported accuracy in [33] is 71.06.
        % ``KD'' means the original knowledge distillation method [15].
        For a fair comparison, we control the cost of all $S_1$ at a similar level.
        Our ResKD can work well with different distillation methods.
        }
        \label{table.KD_method32}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \begin{tabular}{llll}
        \toprule
        KD Method                    & Model    &Accuracy (\%)      & MFLOPs \\
       % \toprule
       % \emph{Teacher} \\
       %                              & Res110   &74.31              & 255.28 \\
        \toprule
        \multicolumn{4}{l}{\emph{Feature Distillation}} \\
        \multirow{2}{*}{FitNet~[21]} & Res32    &70.92 / 71.06 [33] & 69.76\\
                                     & $S_1$    &75.12 (\textcolor{red}{$+$4.20 / $+$4.06})&64.49 (\textcolor{green}{$-$5.27})\\
        \midrule
        \multirow{2}{*}{AT [23]}     & Res32 &72.80 / 72.31 [33]&69.76\\
                                     & $S_1$ &75.65 (\textcolor{red}{$+$2.85 / $+$3.34})&63.74 (\textcolor{green}{$-$6.02})\\
         \midrule
         \multirow{2}{*}{SP [24]}     & Res32 &72.81 / 72.69 [33]&69.76\\
                                      & $S_1$ &75.44 (\textcolor{red}{$+$2.63 / $+$2.75})&63.63 (\textcolor{green}{$-$6.13}) \\
        \midrule
        \multirow{2}{*}{CC [59]}     & Res32 &71.89 / 71.48 [33]&69.76\\
                                     & $S_1$ &75.34 (\textcolor{red}{$+$3.45 / $+$3.86})&65.72 (\textcolor{green}{$-$4.04})  \\
         \midrule
         \multirow{2}{*}{VID [28]}    & Res32 &72.60 / 72.61 [33]&69.76\\
                                      & $S_1$ &76.10 (\textcolor{red}{$+$3.50 / $+$3.49})&63.46 (\textcolor{green}{$-$6.30})\\
        \midrule
        \multirow{2}{*}{RKD [26]}    & Res32 &72.51 / 71.82 [33]&69.76\\
                                     & $S_1$ &75.52 (\textcolor{red}{$+$3.01 / $+$3.70})&64.97 (\textcolor{green}{$-$4.79})\\
        \midrule
        \multirow{2}{*}{PKT [30]}    & Res32 &73.38 / 72.61 [33]&69.76\\
                                     & $S_1$ &75.82 (\textcolor{red}{$+$2.44 / $+$3.21})& 64.02 (\textcolor{green}{$-$5.74})\\
        \midrule
        \multirow{2}{*}{AB [32]}     & Res32 &71.73 / 70.98 [33]&69.76\\
                                     & $S_1$ &77.11 (\textcolor{red}{$+$5.38 / $+$6.13})&  64.75 (\textcolor{green}{$-$5.01})\\
        \midrule
        \multirow{2}{*}{FT [31]}     & Res32 &72.68 / 72.37 [33]&69.76\\
                                     & $S_1$ & 75.78 (\textcolor{red}{$+$3.10 / $+$3.41})& 64.45 (\textcolor{green}{$-$5.31})\\
        \midrule
        \multirow{2}{*}{NST [29]}    & Res32 &72.37 / 71.96 [33]&69.76\\
                                     & $S_1$ & 75.93 (\textcolor{red}{$+$3.56 / $+$3.97})& 64.46 (\textcolor{green}{$-$5.30})\\
        \midrule
        \multirow{2}{*}{CRD [33]}    & Res32 &73.87 / 73.48 [33] &69.76\\
                                     & $S_1$ & 76.07 (\textcolor{red}{$+$2.20 / $+$2.59})& 62.80 (\textcolor{green}{$-$6.96})\\
        \toprule
        \multicolumn{4}{l}{\emph{Both Prediction and Feature Distillation}} \\
        \multirow{2}{*}{CRD+KD [33]} & Res32 &74.40 / 73.75 [33] &69.76\\
                                     & $S_1$ & 75.75  (\textcolor{red}{$+$1.35 / $+$2.00})& 57.37 (\textcolor{green}{$-$12.39})\\


        \bottomrule
        
        \end{tabular}
        
        \end{center}
        \end{table*}

==> minor_sup/tradeoff.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{The comparison of ResKD $S_1$ and relatively big student networks $S_{big}$ with similar cost on CIFAR-100 based on the new code [r1]. $S_1$ (res20-0.75) means we use ResNet-20 whose channels of each layer is 75\% of the original ResNet-20 as $S_0$. 
        WRN-40-2 means the wide residual network whose depth and widening factor is 40 and 2. 
        When we report $S_{big}$ accuracy as 74.03 / 73.08 [48], 74.03 is the result based on our reimplementation, and 73.08 is the result in [48]. 
        We use the original knowledge distillation [15] in this experiment. 
        Our ResKD can lead to a better accuracy-cost trade-off.
        }
        \label{table.tradeoff}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \begin{tabular}{cccc}
            \toprule

        $T$ & $S_{big}$ & ResKD $S_1$  & \\
%        (Ours / Reported)
       Accuracy (\%) & Accuracy (\%) & Accuracy (\%) & Accuracy Gap (\%)  \\
     MFLOPs &  MFLOPs & MFLOPs & MFLOP Gap \\
        \toprule
    %    \multicolumn{5}{l}{\emph{Comparison with Similar Cost but Deeper Network}} \\
        
        ResNet110&ResNet32&$S_1$ (res20) \\
        74.31&74.03 / 73.08 [48]& 75.69 &+1.66 / +2.61 \\
        255.28& 69.76 &  56.96 & -12.80 \\
        \midrule
        ResNet110&ResNet20&$S_1$ (res20-0.75) \\
        74.31&71.03 / 70.67 [48]& 72.18 &+1.15 / + 1.51\\
        255.28& 41.22 &  33.77 & -7.45 \\
        \midrule
        WRN-40-2&WRN-16-2&$S_1$ (WRN-16-1.5) \\
        75.61&75.10 / 74.92 [48]& 76.75 &+1.65 / + 1.83\\
        329.02& 101.61 & 73.20 & -28.41 \\
        \bottomrule
        %
        \end{tabular}
        
        \end{center}
        \end{table*}

==> minor_sup/tradeoff_image.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{
            The comparison of ResKD $S_1$ and the relatively big student network $S_{big}$ with similar cost on ImageNet. $S_1$ (Res18-0.75x) means we use ResNet-18 (0.75x) as $S_0$. 
            ResNet-18 (0.75x) has the same architecture as ResNet-18, and the number of channels of each layer is 75\% of ResNet-18.
            When we report accuracy as 70.02 / 70.40 [44], 70.02 is the result based on our implementation, and 70.40 is the result in [44].
            We use the original knowledge distillation [15] in this experiment. 
            Our ResKD can lead to a better accuracy-cost trade-off based on ImageNet.  
            }
        \label{table.tradeoff_image}

        \begin{tabular}{cccc}
            \toprule

        $T$ & $S_{big}$ & ResKD $S_1$  & \\
        Accuracy (\%) & Accuracy (\%) & Accuracy (\%) & Accuracy Gap (\%)  \\
         MFLOPs &  MFLOPs & MFLOPs & MFLOPs Gap \\
        \toprule
        ResNet50&ResNet18&$S_1$ (Res18-0.75x) \\
        75.50&70.02 / 70.40 [44] & 72.32 &+2.30 / +1.92 \\
        4119& 1821 & 1627  & -194 \\ 
        \bottomrule
        
        \end{tabular}
        
        \end{center}
        \end{table*}

==> minor_sup/tradeoff_imagenew.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{
            The comparison of ResKD $S_1$ and the relatively big student network ResNet-18 with similar cost on ImageNet. $S_1$ (Res18-0.75x) means we use ResNet-18 (0.75x) as $S_0$. 
            ResNet-18 (0.75x) has the same architecture as ResNet-18, and the number of channels of each layer is 75\% of ResNet-18.
            When we report accuracy as 70.02 / 70.40 [27], 70.02 is the result based on our implementation, and 70.40 is the result in [27].
            We use the original knowledge distillation [15] in this experiment. 
            Our ResKD can lead to a better accuracy-cost trade-off based on ImageNet.  
            }
        \label{table.tradeoff_image}

        \begin{tabular}{lcccc}
            \toprule
        

        Models &Accuracy (\%)&Accuracy Gap (\%)&MFLOPs &MFLOPs Gap \\
        \toprule
        \multicolumn{5}{l}{\emph{Teacher}} \\
        Res50&75.50&-&4119&-\\
        \multicolumn{5}{l}{\emph{Students}} \\
        Res18&70.02 / 70.40 [27]&-& 1821&-\\
        $S_1$ (Res18-0.75x)&72.32 &+2.30 / +1.92&1627  & -194 \\ 
        
        % $T$ & $S_{big}$ & ResKD $S_1$  & \\
        % Accuracy (\%) & Accuracy (\%) & Accuracy (\%) & Accuracy Gap (\%)  \\
        %  MFLOPs &  MFLOPs & MFLOPs & MFLOPs Gap \\
        % \toprule
        % ResNet50&ResNet18&$S_1$ (Res18-0.75x) \\
        % 75.50&70.02 / 70.40 [44] & 72.32 &+2.30 / +1.92 \\
        % 4119& 1821 & 1627  & -194 \\ 
        \bottomrule
        
        \end{tabular}
        
        \end{center}
        \end{table*}

==> minor_sup/tradeoffnew.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{\small The comparison of ResKD models to student networks with similar cost on CIFAR-100 and ImageNet based on [r1]. ``$S_1$ (Res20)'' means ResNet-20 is used as $S_0$. ``$S_1$ (Res20-0.75)'' means the tailored ResNet-20 where the  channel number of each layer is 75\% of the original ResNet-20 is used as $S_0$. 
        ``WRN-40-2'' means the wide residual network whose depth and widening factor is 40 and 2. 
        When we report accuracy as ``74.03 / 73.08 [33]'', 74.03 is the result based on our re-implementation, and 73.08 is the result reported in [33]. 
        We use the original knowledge distillation [15] in this experiment. 
        %Our ResKD can lead to a better accuracy-cost trade-off.
        }
        \label{table.tradeoff}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \footnotesize
        \begin{tabular}{clcccc}
        \toprule
        Dataset                    &   Model             &   Accuracy (\%)       &   Accuracy Gap (\%)   &   MFLOPs  &   MFLOPs Gap \\
        \toprule
        \multirow{14}{*}{\rotatebox{90}{CIFAR-100}} % although it only extends 12 rows, we can change the row number to make it more balanced
                                    &   \multicolumn{5}{l}{\emph{Teacher}} \\
                                    &   Res110            &   74.31               &   -                   &   255.28  &   -          \\
                                    &   \multicolumn{5}{l}{\emph{Students}} \\
                                    &   Res32             &   74.03 / 73.08 [33]  &   -                   &   69.76   &   -          \\
                                    &   $S_1$ (Res20)     &   75.69               &   +1.66 / +2.61       &   56.96   &   -12.80     \\
                                    &   Res20             &   71.03 / 70.67 [33]  &   -                   &   41.22   &   -          \\
                                    &   $S_1$ (Res20-0.75)&   72.18               &   +1.15 / +1.51       &   33.77   &   -7.45      \\
                                    \cmidrule{2-6}
                                    &   \multicolumn{5}{l}{\emph{Teacher}} \\
                                    &   WRN-40-2          &   75.61               &   -                   &   329.02  &   -          \\
                                    &   \emph{Students}\\
                                    &   WRN-16-2          &   75.10 / 74.92 [33]  &   -                   &   101.61  &   -          \\
                                    &   $S_1$ (WRN-16-1.5)&   76.75               &   +1.65 / +1.83       &   73.20   &   -28.41     \\
        \midrule
        \multirow{5}{*}{\rotatebox{90}{ImageNet}}   
                                    &   \multicolumn{5}{l}{\emph{Teacher}} \\
                                    &   Res50             &   75.50               &   -                   &   4119    &   -          \\
                                    &   \multicolumn{5}{l}{\emph{Students}} \\
                                    &   Res18             &   70.02 / 70.40 [27]  &   -                   &   1821    &   -          \\
                                    &   $S_1$ (Res18-0.75)&   72.32               &   +2.30 / +1.92       &   1627    &   -194       \\ 
        \bottomrule
        \end{tabular}
        \end{center}
        \end{table*}

        \vspace{-1em}



==> minor_sup/tradeoffv1.tex <==
    \begin{table*}[h]
        \begin{center}
        \caption{The comparison of ResKD $S_1$ and relatively big student networks with similar or less cost on CIFAR-100. $S_1$ (ResNet20) / $S_1$ (Shuffle0.5x) means we use ResNet-20 / ShuffleNetv2 (0.5x) as $S_0$, which is shallower / narrower than ResNet-32 / ShuffleNetv2 (1x). 
        The architectures of $S_0$ and $S_{big}$ is the same in [r1].
        When we report $S_{big}$ accuracy as 74.03 / 73.08, 74.03 is the result based on our reimplementation and 73.08 is the result in other papers. 
        ``KD'' means the original knowledge distillation method [15]. 
        Our ResKD can lead to a better accuracy-cost trade-off based on different KD method.
        }
        \label{table.tradeoff}
        %
        %\checkmark
        %\multirow{3}{*}{Knowledge}
        \begin{tabular}{ccccc}
            \toprule

        Knowledge& $T$ & $S_{big}$ & ResKD $S_1$  & \\
%        (Ours / Reported)
        Distillation& Accuracy (\%) & Accuracy (\%) & Accuracy (\%) & Accuracy Gap (\%)  \\
        Method&  MFlops &  MFlops & MFlops & MFlops Gap \\
        \toprule
    %    \multicolumn{5}{l}{\emph{Comparison with Similar Cost but Deeper Network}} \\
        
        \multirow{3}{*}{KD}&ResNet110&ResNet32&$S_1$ (ResNet20) \\
        &74.31&74.03 / 73.08 [r2]& 75.87 &+1.84 / +2.79 \\
        &255& 70 &  60 & -10 \\
        \toprule
        \multirow{3}{*}{CRD}& ResNet110&ResNet32&$S_1$ (ResNet20) \\
        &74.31&73.87 / 73.48 [r2]& xxxxx &+xxx \\
        &255& 70 & xxxxx  & -xxxx \\
        \toprule
    %    \multicolumn{5}{c}{\textbf{Comparison with Similar Cost but Wider Network}} \\
    %    \toprule
        \multirow{3}{*}{KD}&resnet32x4&ShuffleNetV2 (1x)&$S_1$ (Shuffle0.5x) \\
        &79.42&75.59 / 74.45 [r2]& xxxxx &+xxx \\
        &1086& 46 & xxxxx  & -xxxx \\
        \toprule
        \multirow{3}{*}{CRD}& resnet32x4&ShuffleNetV2 (1x)&$S_1$ (Shuffle0.5x) \\
        &79.42&75.63 / 75.65 [r2]& xxxxx &+xxx \\
        &1086& 46 & xxxxx  & -xxxx \\
        \bottomrule
        
        \end{tabular}
        
        \end{center}
        \end{table*}

==> rebuttal_section/r1.tex <==
\large{\textbf{\centerline{Reviewer 1}}}

\begin{qanda}
   
\Q This approach is described as novel in the area of knowledge distillation e.g. ``the discrepancy between a teacher and a student can be considered as knowledge, and it remains relatively unexplored.'' However, learning the residual between groundtruth (the outputs of the teacher can be regarded groundtruth in this paper) and prediction is totally a common way for face alignment. As such, the discussion should be added to show the specific in the area of knowledge distillation.

%\A The specific area of knowledge distillation for residual-guided is that all images are always considered in a certain domain and the well-trained learning target $T$ is given through the training period, but the student network also has the performance gap compared with $T$. It is different from face alignment whose performance gap is caused by different inputs, which have large pose variations or large degree rotation compared with training images (just like two domains).
%The student, $S_0$, cannot learn the target well due to the scale and ability of itself instead of the change of input. To solve this limitation, we employ $R_1$ to bridge the gap between $T$ and $S_0$.

\A The specific area of our ResKD in knowledge distillation is that: our res-student is a supplement to $S_0$ to improve its ability instead of doing a refinement on the output of $S_0$ to approach ground truth. 

\ \ \ \ In detail, our pipeline is different from face alignment in the following aspects. 

\ \ \ \ Firstly, $S_0$ and all $R_i$ in our ResKD only take the original image as input and output logits while the regressors in face alignment mostly take the original image and the current landmark \cite{park2020acn}, \cite{cao2014face}, \cite{ren2014face}, \cite{zhu2016face}, shape estimation \cite{yang2017stacked} or heatmap \cite{wan2020robust} as two inputs. The calculation of each $R_i$ in residual knowledge distillation is independent when evaluating and the results of former $S_{i-1}$ are only needed in sample-adaptive inference for determining whether the current $R_i$ is necessary. 

\ \ \ \ Secondly, the supervision of our res-student is not only the final output of $T$ but also other information about $T$. E.g. the information can be some middle layers output of the current input image of $T$ \cite{park2019relational} or some information between the samples in the current batch \cite{peng2019correlation}, which is determined by the knowledge distillation method we use. In our manuscript, we do the experiment combined with RKD \cite{park2019relational} using the feature of some middle layers as well as normal KD using the final output of $T$.

 %learning the residual in face alignment is needed because different inputs, which have large pose variations or large degree rotation compared with each other when the student network in ResKD is limited by the scale and generalization of itself compared with $T$. For this difference, the regressors in face alignment mostly use landmark \cite{park2020acn}, \cite{cao2014face}, \cite{ren2014face}, \cite{zhu2016face}, shape estimation \cite{yang2017stacked} or heatmap \cite{wan2020robust} of the current input image when our ResKD can use not only the logits or the outputs of some middle layers of the current input image but also some information between the samples in the current batch \cite{peng2019correlation}, which is determined by the knowledge distillation method we use. In our manuscript, we do the experiment combined with RKD using the feature of some middle layers as well as normal KD using the logits.



%Secondly, the face alignment mostly uses the original image and landmark~\cite{park2020acn},~\cite{cao2014face}, \cite{ren2014face}, \cite{zhu2016face}, shape estimation \cite{yang2017stacked}, or heatmap \cite{wan2020robust}, which is the output of certain locations. Our ResKD can not only use the final result, logits, but also the feature, the outputs of some middle layers, etc, which is divided by the knowledge distillation method we use. In our manuscript, we do the experiment combined with RKD using the feature of some middle layers as well as normal KD using the logits.

\ \ \ \ Also, our ResKD mostly focuses on image classification having less prior (e.g. the structure of landmark \cite{cootes1995active}, \cite{cootes1998active}) instead of face alignment. 
 

%\input{rebuttal_sup/vgg_inceptionimage.tex}

\Q There should be a specific subsection in the result section, showing the impact of the hyper-parameter THenergy on the final results.

\A  Following your suggestion, we have added the following discussion to Sec. IV.C of the revised manuscript.

%\begin{figure}[tb]
%	\centering
%	\includegraphics[width=0.5\linewidth]{figures/TH.pdf}
%	\caption{The relationship between the cost reduction of $R_1$ and $\mathrm{TH}_{\mathrm{energy}}$ on  both validation set and test set on CIFAR-100. $T$ is ResNet-110, $S_0$ is ResNet-20, and $R_{1}$ is ResNet-14. The result indicates that it is reasonable to calculate  $\mathrm{TH}_{\mathrm{energy}}$ on a validation set for the sample-adaptive strategy. }
%	\label{THfig}
%\end{figure}

%-------------------------------------------------------------------------

\begin{figure}[h]
%\centering  
\subfigure[]{
    \begin{minipage}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{rebuttal_sup/TH_100.pdf}\\
        %\vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
%    \caption{Relationship between $R_1$'s cost and $S_1$'s performance.}
    \label{THREa}
}
\subfigure[]{
    \begin{minipage}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{rebuttal_sup/TH_imagenet.pdf}\\
        %\vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
    \label{THREb}
}
\subfigure[]{
    \begin{minipage}[t]{0.3\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/TH.pdf}\\
        %\vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
    \label{THREc}
}

\centering
\caption{This figure shows the results about $\mathrm{TH}_{\mathrm{energy}}$.
(a) and (b) indicate the relationship between the cost reduction of $R_1$ and performance of $S_1$ according to $\mathrm{TH}_{\mathrm{energy}}$ on test set on CIFAR-100 / ImageNet. 
For CIFAR-100, $T$ is ResNet-110, $S_0$ is ResNet-20, and $R_{1}$ is ResNet-14. For ImageNet, $T$ is ResNet-50, $S_0$ is ResNet-18, and $R_{1}$ is a NAS-based architecture. The result indicates that our trade-off is done by our sample-adaptive strategy. 
For (c), the relationship between the cost reduction of $R_1$ and $\mathrm{TH}_{\mathrm{energy}}$ on both validation set and test set on CIFAR-100 is shown. 
$T$ is ResNet-110, $S_0$ is ResNet-20, and $R_{1}$ is ResNet-14. 
The result indicates that it is reasonable to calculate  $\mathrm{TH}_{\mathrm{energy}}$ on a validation set for the sample-adaptive strategy.
}
%\vspace{-0.2cm}
\label{THRE}
\end{figure}


\ \ \ \ \emph{In addition, we carry out more experiments and analysis on our sample-adaptive strategy. We pay attention to the trade-off between performance and cost. We do this ablation study on CIFAR-100. In Fig. \ref{THRE} (a), the relation between performance of $S_1$ and the cost of $R_1$ is showed. With the $\mathrm{TH}_{\mathrm{energy}}$  decreasing, the performance goes down slowly at first when the cost reduces rapidly at the beginning. Based on this observation, we set $\mathrm{TH}_{\mathrm{energy}}$ as 90\% of the $S_1$'s on the validation set, a subset of the training set.}

\ \ \ \ \emph{Besides, we also validate our observation on ImageNet in Fig. \ref{THRE} (b). The results are similar.}


\input{rebuttal_sup/vgg_inceptioncifar.tex}


\Q This paper describes that this approach is generic to knowledge distillation methods. However, this claim does not feel backed up very much by the experiments later in the paper. Instead, one experiment is run to convince the reader that: DML and RKD with residual-guided learning are taken to be comparison, but all the methods are based on ResNet. More architectures, such as VGG or Inception, should be discussed in experiment section.

%and Table \ref{vgg_inception_image}
\A Following your suggestion, we add some experiments for more backbones to show our ResKD is generic to different backbones. As shown in Table \ref{vgg_inception_cifar}, our pipeline can be used with different backbones (e.g. VGG, Inceptionv3, Xception, mobilenetv2 and shufflenetv2) on CIFAR-10 / 100. 

\ \ \ \ Based on the results, our ResKD is generic to different backbones in knowledge distillation. We have added \ref{vgg_inception_cifar} to Sec. IV.C of the revised manuscript.

%\bibliographystyle{alpha}
%\bibliography{IEEEabrv,bibli_rebuttal_1}


\end{qanda}
\newpage






==> rebuttal_section/r2.tex <==
\large{\textbf{\centerline{Reviewer 2}}}
\begin{qanda}
    \Q In Fig. 1, ``Training stage 0'' in the middle figure should be ``Training stage 1''; 

    \A  Following your suggestion, We have fixed the typo in Fig. 1 in the revised manuscript. 
    
    \begin{figure}[h]
        %\centering 
        \subfigure[]{
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \includegraphics[width=1\linewidth]{rebuttal_sup/T_20.pdf}\\
                %\vspace{0.02cm}
                %\caption{fig1}
            \end{minipage}%
            \label{20ttaua}
        }
        \subfigure[]{
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \includegraphics[width=1\linewidth]{rebuttal_sup/tau_20.pdf}\\
                %\vspace{0.02cm}
                %\caption{fig1}
            \end{minipage}%
            \label{20ttaub}
        }     
        \subfigure[]{
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \includegraphics[width=1\linewidth]{rebuttal_sup/T_20_14.pdf}\\
                %\vspace{0.02cm}
                %\caption{fig1}
            \end{minipage}%
            \label{20ttauc}
        }
        \subfigure[]{
            \begin{minipage}[t]{0.45\linewidth}
                \centering
                \includegraphics[width=1\linewidth]{rebuttal_sup/tau_20_14.pdf}\\
                %\vspace{0.02cm}
                %\caption{fig1}
            \end{minipage}%
            \label{20ttaud}
        }
        \centering
        \caption{The relationship between hyper-parameters ($\tau$ and t) and the performance of $S_0$ and $S_1$ on CIFAR-100. $T$ is ResNet-110, $S_0$ is ResNet-20, and $R_{1}$ is ResNet-14 The result indicates that these hyper-parameters can partly affect the final performance but not large.}
        %\vspace{-0.2cm}
        \label{20ttau}
        \end{figure}


    \Q Why is STACNAS [44] selected to obtain the final suitable network? 

    \A Firstly, because adding the knowledge distillation as a loss term in the search period, we employ a NAS method that has continuous architecture parameters. 

    \ \ \ \ Secondly, We select STACNAS from many continuous architecture parameters NAS methods because it can reduce the searching stage cost when using the same searching space by using a two-stage searching instead of the original searching stage. In detail, we choose the kind of layers in stage 1 from Max pooling $3 \times 3$, SkipConnect, Conv $3 \times 3$, DilConv $3 \times 3$ etc. when we choose the accurate kind for a certain layer in stage 2. (e.g. when a SepConv  $3 \times 3$ layer is selected in stage 1, we will select the final one from SepConv $3 \times 3$ and SepConv $5 \times 5$ in stage 2.)
%    \A Because we add the knowledge distillation in the search period, we need a NAS method that have continuous architecture parameters. We compare three NAS method and select STACNAS [44] finally. Our method is also generic to different NAS methods and Table \ref{three_NAS} shows three different NAS methods on CIFAR-100. 

%\input{rebuttal_sup/NAS.tex}

    \Q How to set hyper-parameters $\tau$ and t of Equation (3) in experiments? 
      
%        \begin{figure}[tb]
%        %\centering 
%        \subfigure[]{
%            \begin{minipage}[t]{0.5\linewidth}
%                \centering
%                \includegraphics[width=1\linewidth]{rebuttal_sup/T_20_14.pdf}\\
%                %\vspace{0.02cm}
%                %\caption{fig1}
%            \end{minipage}%
%        }
%        \subfigure[]{
%            \begin{minipage}[t]{0.5\linewidth}
%                \centering
%                \includegraphics[width=1\linewidth]{rebuttal_sup/tau_20_14.pdf}\\
%                %\vspace{0.02cm}
%                %\caption{fig1}
%            \end{minipage}%
%        }
        
%        \centering
%        \caption{The relationship between the performance of $S_0$ and t and $\tau$ on the test set on CIFAR-100. $T$ is ResNet-110, $S_0$ is ResNet-20, and $R_{1}$ is ResNet-14 The result indicates that these hyper-parameters can partly affect the final performance but not large.}
%        %\vspace{-0.2cm}
%        \label{20_14ttau}
%        \end{figure}

    \A For the t of our student network, we use similar settings as \cite{yuan2020revisiting} which means $\tau = 0.9 / 0.5 / 0.5 / 0.1$ for $S_0$ on CIFAR-10 / CIFAR-100 / Tiny-ImageNet / ImageNet when $\tau = 0.1$ for $R_1$ on all datasets.
    We set $t = 20$ in all situations. 
    
    \ \ \ \ TO better solve your concern, we have added the experiments on CIFAR-10 / 100 to show the influence of t and $\tau$. 

    \ \ \ \ Extra experiments on CIFAR-10 / 100 to show the influence of t and $\tau$ are added in Fig. \ref{20ttau}. 
    The results about t for $S_0$ are summarized in Fig. \ref{20ttau} (a) and the results about t for $R_1$ are summarized in Fig. \ref{20ttau} (c). 
    The results about $\tau$ for $S_0$ are summarized in Fig. \ref{20ttau} (b) and the results about $\tau$ for $R_1$ are summarized in Fig. \ref{20ttau} (d).  

    \ \ \ \ From our additional experiments above, we can learn that t and  $\tau$ can partly affect the final performance but not large.
    We report the best in our manuscript and the additional experiments are also added to Sec. IV.B of the revised manuscript.


    \Q A reference on transfer learning could be cited in the paper: Hu et al., Deep transfer metric learning, IEEE TIP, 2016. Overall, the novelty and contribution of this paper is significant, and the experimental evaluation is sufficient.

    \A  Following your suggestion, we have added the reference you recommended to Sec. V of the revised manuscript.

%\bibliographystyle{alpha}
%\bibliography{IEEEabrv,bibli_rebuttal_2}

\end{qanda}

\newpage


==> rebuttal_section/r3.tex <==
\large{\textbf{\centerline{Reviewer 3}}}

\begin{qanda}

    \Q This paper failed to clearly verify the proposed method. This paper didn't compare with any previous state-of-the-art method, which makes it hard to judge the contribution of this paper. The results of the baseline student model reported in this paper are significantly lower than previous works. For example, the ResNet-18 (a.k.a. ResNet-20) should achieve ~75\% performance on CIFAR-10 as reported in \cite{yuan2020revisiting} and many other works. But the distilled ResNet-18 in this paper can only achieve 74.06\%, which indicates the implementation of this paper may be problematic and thus makes the results reported in this paper unconvincing. \cite{yuan2020revisiting} Revisiting Knowledge Distillation via Label Smoothing Regularization, CVPR 2020.

    \A For your concern about ResNet-20 and ResNet-18, we explain it in three aspects: the difference of architecture, performance, and cost. 
    
    \ \ \ \ The architecture of ResNet-20 is similar to ResNet-18's, but the width of them is different, and ResNet-18 is much wider than ResNet-20.
    After we carefully check the original ResNet paper and the paper you recommend, ResNet-18 in \cite{yuan2020revisiting} is based on the network proposed in Sec.4.1 and Table. 1 in \cite{he2016deep} and is summarized in Fig \ref{difference} left while ResNet-20 is based on Sec.4.2 and Table. 6 in \cite{he2016deep} and is summarized in Fig \ref{difference} right. This Figure is build similarly as the Fig. 3 in \cite{he2016deep}. 

    \ \ \ \ In brief, ResNet-18 has 17 convolution layers and a fully-connect layer, 11.22M parameters, and 557M FLOPs for a single CIFAR-100 sample while  ResNet-20 has 19 convolution layers and a fully-connect layer,  0.28M parameters and 41M FLOPs in CIFAR-100 experiment with input images size $32 \times 32$.

    \ \ \ \ Secondly, the performance of  ResNet-18 and  ResNet-20 reported in papers are different. The performance of ResNet-18 with knowledge distillation  in \cite{yuan2020revisiting} is reported as 75.87\% just like your opinion: ResNet-18 should achieve about 75\% performance on CIFAR-100. The performance of ResNet-20 with knowledge distillation in \cite{peng2019correlation}, \cite{dabouei2020supermix}, \cite{xu2020knowledge} is reported as 70.80\%, 70.67\%, 70.66\%, which is the same level as our results, ResNet-20 should achieve ~70\% performance on CIFAR-100.
    The about 0.7\% gap for ResNet-20 is caused by the difference in image preprocessing: we follow the image preprocessing of CIFAR-10 in \cite{he2016deep} that does not employ a 15-degree random rotation for training image when \cite{peng2019correlation}, \cite{dabouei2020supermix} and \cite{xu2020knowledge} employ it. 

    \ \ \ \ In addition, we also follow the settings in \cite{yuan2020revisiting} do experiments besides ResNet-50 / ResNet-18 and observe the influence of random rotation for ResNet-110 / ResNet-20,  which are summarized in Table \ref{50_18_r3}. We can learn that the ResNet-18 has much better performance than ResNet-20 as well as ResNet-18 needs much more cost. Also, we show other results of \cite{yuan2020revisiting} settings (e.g. ResNet-50 and MobileNetv2) and compared with \cite{yuan2020revisiting} or other paper.
\input{rebuttal_sup/R3_50_18.tex}
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.5\linewidth]{rebuttal_sup/rebuttal_18_20.pdf}
	\caption{The difference between ResNet-18 and ResNet-20. The left one is ResNet-18, and the right one is ResNet-20. }
	\label{difference}
\end{figure}

    Our ResKD is generic to knowledge distillation methods, besides state-of-the-art methods. In Table IV of our paper, we combine DML and RKD with our ResKD. 
    We also combine our ResKD with the method you recommend, the results are summarized in Table \ref{SOTA}.
\input{rebuttal_sup/SOTA.tex} 
%[16] B. Peng, X. Jin, J. Liu, D. Li, Y. Wu, Y. Liu, S. Zhou, and Z. Zhang. Correlation congruence for knowledge distillation, in Proc.ICCV, 2019, pp. 5007–5016.


%[r1] Yuan L, Tay F E H, Li G, et al. Revisiting Knowledge Distillation via Label Smoothing Regularization, in Proc. CVPR, 2020, pp. 3903-3911.

%[r2] Dabouei A, Soleymani S, Taherkhani F, et al. SuperMix: Supervising the Mixing Data Augmentation, arXiv preprint arXiv:2003.05034, 2020.

%[r3] Xu G, Liu Z, Li X, et al. Knowledge distillation meets self-supervision, ECCV, 2020, pp. 588-604.

%[r4] Walawalkar D, Shen Z, Savvides M. Online Ensemble Model Compression using Knowledge Distillation, ECCV,2020, pp. 18-35.




    \Q The improvement on ImageNet is quite incremental (more FLOPs compared to $S_0$, 1-2\% improvement). Since results on CIFAR-10/100 may not precisely reflect the actual performance of the method, the effectiveness of the method may be questionable.

    \A The questions about CIFAR-100 experiments are explained in the former answer.

    \ \ \ \ For your incremental improvement concern, based on knowledge distillation is aimed at balancing between performance and cost (e.g. FLOPS) of the student network. Our goal is to improve the student network performance (e.g. 1-2\% improvement on ImageNet) with little extra cost. For example, in the ImageNet setting, we improve the ResNet-18 requiring 1821M FLOPs 1.35\% with only 395M FLOPs extra cost. The balance of trade-off is controlled by the choice of each res-students. The related experiments are shown in Table III in our paper. 
    Also, if a better performance is needed, we can use a larger $R_1$ just as $S_1$ (large) in \cref{SOTA} and $S_1$ (18-L) in \cref{50_18_r3}. if a lower cost is needed, we can use a smaller $R_1$ just as $S_1$ (small) in \cref{SOTA} and $S_1$ (18-S) in \cref{50_18_r3}. 

%\bibliographystyle{alpha}
%\bibliography{IEEEabrv,bibli_rebuttal_3}

\end{qanda}


==> rebuttal_sup/18_use.tex <==
\begin{table*}[h]
\begin{center}
\caption{Results about ResNet-18 on CIFAR-100. $T$ is ResNet-50, $S_0$ is ResNet-18, and $R_1$ is a NAS-based network.}
\label{18_use}
\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & Teacher & SA &  Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Baseline}  &  & & & &\\
ResNet50& - & & 78.21 & 23.71 &  1306  \\
ResNet50\cite{yuan2020revisiting}& - & & 78.16 & 23.71 & 1306   \\
ResNet18& - & & 76.80 & 11.22 & 557   \\
ResNet18\cite{yuan2020revisiting}& - & & 75.87 &   11.22 & 557   \\

\midrule
\emph{Students}  & & & & \\
ResNet18& ResNet50 & & 78.67 &  11.22 & 557  \\

\midrule
\emph{ResKD students} & & & & &\\
$S_1$ (18-S) & ResNet50 &  & 80.05 &  11.58 & 620    \\
$S_1$ (18-S)& ResNet50 & $\checkmark$ & 80.08 & 11.58 & 576 \\
\bottomrule
\end{tabular}

\end{center}
\end{table*}




==> rebuttal_sup/NAS.tex <==
\begin{table*}[tb]
\begin{center}
\caption{
aaaaaa
    }
\label{three_NAS}

\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & Optimizer & SA & Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Teacher}  & & & & &\\
Res110 & SGD &  & 72.44 & 1.734 &  255\\
\midrule
\emph{Students}  & & & & &\\
Res20 & KD &  & 70.09 & 0.276 &  41\\

\midrule
\emph{ResKD students}  & & & & &\\


STACNAS  & KD &  & 74.06 & 0.485 &  81\\
STACNAS  & KD & $\checkmark$ & 74.06 &  0.485 &  59\\
DARTS  & KD &  &  &  & \\
DARTS  & KD & $\checkmark$ &  &   &  \\
PC-DARTS  & KD &  &  &  &  \\
PC-DARTS  & KD & $\checkmark$ &  &   &  \\
\bottomrule
\end{tabular}

\end{center}
\end{table*}



==> rebuttal_sup/R3_50_18.tex <==
\begin{table*}[tb]
\begin{center}
\caption{Different results on CIFAR-100. For ResNet-110 / ResNet-20, * means taking the 15-degree random rotation into account as \cite{yuan2020revisiting}. The ResNet20* is taught by ResNet110*. 
$S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is MobileNetv2 / ShuffleNetv2 when $R_1$ is a NAS-based network.
$S_0$ of $S_1$ (18-L) and $S_1$ (18-S) is ResNet18. 
$S_1$ (18-L) means we use a larger NAS-based network $R_1$ to achieve a better performance when $S_1$ (18-L) means we use a smaller NAS-based network $R_1$ to cost less. 
    }
\label{50_18_r3}

\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & Teacher & SA &  Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Baseline}  &  & & & &\\
ResNet50& - & & 78.21 & 23.71 &  1306  \\
ResNet50\cite{yuan2020revisiting}& - & & 78.16 & 23.71 & 1306   \\
ResNet18& - & & 76.80 & 11.22 & 557   \\
ResNet18\cite{yuan2020revisiting}& - & & 75.87 &   11.22 & 557   \\
MobileNetv2& - & & 69.30 & 2.37 &  68  \\
MobileNetv2\cite{yuan2020revisiting}& - & & 68.38  & 2.37 &  68  \\
ShuffleNetv2& - & & 71.52 & 1.36 &  46   \\
ShuffleNetv2\cite{yuan2020revisiting}& - & & 70.34  &   1.36 &  46   \\
ResNet110& - & & 72.44 & 1.73 &  255   \\
ResNet110 \cite{walawalkar2020online}& - & & 72.64 &  1.73 &  255\\
ResNet110*& -&  & 73.23 & 1.73 &  255   \\
\midrule
\emph{Students}  & & & & \\
ResNet20& ResNet110& & 70.09 & 0.28 &  41  \\
ResNet20*& ResNet110*& & 70.88 &  0.28 &  41     \\
ResNet20* \cite{peng2019correlation}& ResNet110*& & 70.80 &  0.28 &  41 \\
ResNet18& ResNet50 & & 78.67 &  11.22 & 557  \\
MobileNetv2& ResNet50 & & 75.31 &  2.37 &  68   \\
MobileNetv2\cite{yuan2020revisiting}& ResNet50&  & 71.04 & 2.37 &  68  \\
ShuffleNetv2& ResNet50&  & 75.92 &   1.36 &  46 \\
ShuffleNetv2\cite{yuan2020revisiting}& ResNet50 & & 72.15 &   1.36 &  46  \\
\midrule
\emph{ResKD students} & & & & &\\
$S_1$ (18-L) & ResNet50 & & 82.67 & 16.04 & 1307    \\
$S_1$ (18-L)& ResNet50 & $\checkmark$ & 82.37 & 16.04 & 785  \\
$S_1$ (18-S) & ResNet50 &  & 80.05 &  11.58 & 620    \\
$S_1$ (18-S)& ResNet50 & $\checkmark$ & 80.08 & 11.58 & 576 \\
$S_1$ (Mobile)& ResNet50 & & 78.67 & 3.13 & 197 \\
$S_1$ (Mobile)& ResNet50 & $\checkmark$ & 78.30 & 3.13  & 101 \\
$S_1$ (Shuffle)& ResNet50 &  & 78.64 & 1.72 & 109 \\
$S_1$ (Shuffle)& ResNet50 & $\checkmark$ & 78.57 & 1.72  & 65 \\
\bottomrule
\end{tabular}

\end{center}
\end{table*}




==> rebuttal_sup/R3_50_18_new.tex <==
\begin{table*}[h]
\begin{center}
\caption{Different results on CIFAR-100. $T$ is ResNet-50 or pt-Res50 (the poor trained ResNet-50 in De-KD), and $S_1$ (Mobile) / $S_1$ (Shuffle) / $S_1$ (pt-Res50) means $R_1$ is a NAS-based network when $S_0$ is MobileNetv2 / ShuffleNetv2 / ResNet-18. ours / [44] is the results we implemented / the results reported in [44].
Our ResKD can improve the performance of different $S_0$ and different KD method and achieve the performance of $T$ with little cost.  \textbf{Bold}: The best results out of students.}
\label{table.50_18_r3}
%
\begin{tabular}{lcccccc}
    \toprule
%\checkmark
\multirow{2}{*}{Architecture}&\multirow{2}{*}{Optimizer} & \multirow{2}{*}{Teacher} & \multirow{2}{*}{Acc.~(\%)} & Acc. gap to $S_0$ & \multirow{2}{*}{MFLOPs} & additional\\
 & &  & & (ours / reported)& & FLOPs to $S_0$\\
\toprule
\textbf{Teachers} \\
ResNet50&SGD& - & 78.21  &- & 1306  &-\\
pt-Res50& SGD & - & 46.92  &- & 1306  &-\\
\toprule
\textbf{Students} \\
MobileNetv2 (ours / [44])&normal KD& ResNet50 &75.31 / 71.04& -& 68 &- \\
$S_1$ (Mobile)&normal KD& ResNet50 & 78.30 & \textbf{+2.99 / +7.26} & 101&  +33\\
\midrule


ShuffleNetv2 (ours / [44])&normal KD& ResNet50 &75.92 / 72.15 & -& 46 &-\\
$S_1$ (Shuffle)& normal KD&ResNet50 & 78.57 & +2.65 / +6.42 & 65 & \textbf{+19} \\

\midrule



ResNet18 (ours / [44])& De-KD&pt-Res50 & 77.54 / 77.23 &  -& 557 &- \\

$S_1$ (pt-Res50)& De-KD&pt-Res50 & 78.91 &+1.37 / +1.68 & 576 & \textbf{+19}\\
\bottomrule

\end{tabular}

\end{center}
\end{table*}
%$S_1$ (18)& normal KD&ResNet50 & 80.08 &+1.41 / +3.21& 576& \textbf{+19}\\


%MobileNetv2& SGD &- & 69.30 & -& 68 &- \\
%MobileNetv2 &normal KD& ResNet50 &71.04& -& 68 & -\\

%ShuffleNetv2& SGD &- &71.52 &- & 46 & - \\
%ShuffleNetv2 [44]& normal KD&ResNet50 &72.15 & -& 46 &-\\

%ResNet18 [44]& SGD  & - & 75.87 & - & 557 &-  \\
%ResNet18 [44]& De-KD&pt-Res50 & 77.23 &  -& 557 &- \\
%$S_1$ (big)& De-KD&pt-Res50 & 81.74 & \textbf{+4.94 / +5.87} & 788 & +231\\

% \begin{table*}[tb]
%     \begin{center}
%     \caption{Different results on CIFAR-100. For ResNet-110 / ResNet-20, * means taking the 15-degree random rotation into account as \cite{yuan2020revisiting}. The ResNet20* is taught by ResNet110*. 
%     $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is MobileNetv2 / ShuffleNetv2 when $R_1$ is a NAS-based network.
%     $S_0$ of $S_1$ (18-L) and $S_1$ (18-S) is ResNet18. 
%     $S_1$ (18-L) means we use a larger NAS-based network $R_1$ to achieve a better performance when $S_1$ (18-L) means we use a smaller NAS-based network $R_1$ to cost less. 
%         }
%     \label{50_18_r3}
    
%     \begin{tabular}{lccccc}
%         \toprule
%     %\checkmark
%     Architecture & Teacher & SA &  Acc.~(\%) & \#Params (M) & MFLOPs\\
%     \midrule
%     \emph{Baseline}  &  & & & &\\
%     ResNet50& - & & 78.21 & 23.71 &  1306  \\
%     ResNet50\cite{yuan2020revisiting}& - & & 78.16 & 23.71 & 1306   \\
%     ResNet18& - & & 76.80 & 11.22 & 557   \\
%     ResNet18\cite{yuan2020revisiting}& - & & 75.87 &   11.22 & 557   \\
%     MobileNetv2& - & & 69.30 & 2.37 &  68  \\
%     MobileNetv2\cite{yuan2020revisiting}& - & & 68.38  & 2.37 &  68  \\
%     ShuffleNetv2& - & & 71.52 & 1.36 &  46   \\
%     ShuffleNetv2\cite{yuan2020revisiting}& - & & 70.34  &   1.36 &  46   \\
%     ResNet110& - & & 72.44 & 1.73 &  255   \\
%     ResNet110 \cite{walawalkar2020online}& - & & 72.64 &  1.73 &  255\\
%     ResNet110*& -&  & 73.23 & 1.73 &  255   \\
%     \midrule
%     \emph{Students}  & & & & \\
%     ResNet20& ResNet110& & 70.09 & 0.28 &  41  \\
%     ResNet20*& ResNet110*& & 70.88 &  0.28 &  41     \\
%     ResNet20* \cite{peng2019correlation}& ResNet110*& & 70.80 &  0.28 &  41 \\
%     ResNet18& ResNet50 & & 78.67 &  11.22 & 557  \\
%     MobileNetv2& ResNet50 & & 75.31 &  2.37 &  68   \\
%     MobileNetv2\cite{yuan2020revisiting}& ResNet50&  & 71.04 & 2.37 &  68  \\
%     ShuffleNetv2& ResNet50&  & 75.92 &   1.36 &  46 \\
%     ShuffleNetv2\cite{yuan2020revisiting}& ResNet50 & & 72.15 &   1.36 &  46  \\
%     \midrule
%     \emph{ResKD students} & & & & &\\
%     $S_1$ (18-L) & ResNet50 & & 82.67 & 16.04 & 1307    \\
%     $S_1$ (18-L)& ResNet50 & $\checkmark$ & 82.37 & 16.04 & 785  \\
%     $S_1$ (18-S) & ResNet50 &  & 80.05 &  11.58 & 620    \\
%     $S_1$ (18-S)& ResNet50 & $\checkmark$ & 80.08 & 11.58 & 576 \\
%     $S_1$ (Mobile)& ResNet50 & & 78.67 & 3.13 & 197 \\
%     $S_1$ (Mobile)& ResNet50 & $\checkmark$ & 78.30 & 3.13  & 101 \\
%     $S_1$ (Shuffle)& ResNet50 &  & 78.64 & 1.72 & 109 \\
%     $S_1$ (Shuffle)& ResNet50 & $\checkmark$ & 78.57 & 1.72  & 65 \\
%     \bottomrule
%     \end{tabular}
    
%     \end{center}
%     \end{table*}
    
    
% \begin{table*}
%     \centering
%     \caption{Experimental results on A, B, and C databases in terms of average MAE.}
%     \begin{tabular}{|c |c |c |c |c | c | c | c | c | c | c| c| c| c|}
%     \hline {Dataset} & {\diagbox{$\alpha$}{$\sigma_s$}} &{1} & {3} & {5} & {7} & {10} \\
%     \hline
     
%     \multirow{5}{*}{A} 
%     & {40} & {0.1703} & {0.1406} & {0.1447} & {0.1078} & {0.0585}   \\
%     \cline{2-7}
%     & {50} & {0.5006} & {0.5360} & {0.3602} & {0.5401} & {0.7303} \\
%     \cline{2-7}
%     & {60} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {70} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {80} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \hline
     
%     \multirow{5}{*}{B} 
%     & {40} & {0.1484} & {0.1406} & {0.1447} & {0.1078} & {0.0585}   \\
%     \cline{2-7}
%     & {50} & {0.5006} & {0.5360} & {0.3602} & {0.5401} & {0.7303} \\
%     \cline{2-7}
%     & {60} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {70} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {80} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \hline
     
%     \multirow{5}{*}{C} 
%     & {40} & {0.1484} & {0.1406} & {0.1447} & {0.1078} & {0.0585}   \\
%     \cline{2-7}
%     & {50} & {0.5006} & {0.5360} & {0.3602} & {0.5401} & {0.7303} \\
%     \cline{2-7}
%     & {60} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {70} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {80} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \hline
     
%     \hline \end{tabular}
%     \label{tab}
%     \end{table*}


% \begin{tabular}{|c|c|c|c|c|}
%     \toprule
% %\checkmark
% Teacher& $S_0$ baseline & $S_0$ (MFLOPs) &  $S_1$ (MFLOPs)&ACC. compared with $S_0$ \\
% ACC. (\%) & ACC.(\%) &ACC. (\%)  &  ACC. (\%)  & ACC. compared with $T$   \\
% MFLOPs & MFLOPs &MFLOPs  &  MFLOPs  & FLOP Percentage of $T$ \\
% \midrule
% %\emph{Baseline}  &  & & & &\\
% & ResNet-18& ResNet-18  & $S_1-18$   &  +1.41\% \\
% &76.80 (75.87\cite{yuan2020revisiting}) &78.67 & 80.08& \textbf{+1.87} (\textbf{+1.92}\cite{yuan2020revisiting})\textbf{\%} \\
% &557 &557& 576& 44.1\%\\
% \cline{2-5}
% ResNet50&MobileNetv2& MobileNetv2& $S_1-Mobile$& \textbf{+2.99} (\textbf{+7.26}\cite{yuan2020revisiting})\textbf{\%}\\
% 78.21(78.16\cite{yuan2020revisiting})&69.30 (68.38 \cite{yuan2020revisiting})& 75.31 (71.04\cite{yuan2020revisiting})& 78.30  & +0.09 (+0.14\cite{yuan2020revisiting})\% \\
% 1306&68& 68& 101 & 7.7\% \\
% \cline{2-5}
% &ShuffleNetv2 & ShuffleNetv2 & $S_1-Shuffle$& +2.65 (+6.42\cite{yuan2020revisiting})\\
% &71.52 (70.34\cite{yuan2020revisiting})& 75.92 (72.15\cite{yuan2020revisiting}) & 78.57 & +0.36 (+0.41\cite{yuan2020revisiting}) \\
% &46& 46& 65& \textbf{5.0\%}\\
% \bottomrule
% \end{tabular}

==> rebuttal_sup/R3_Q1.tex <==
\begin{table*}[h]
\begin{center}
\caption{Performance of distilled ResNet-20 and distilled ResNet-18 on CIFAR-100. The minor performance difference among ResNet-20 of different sources is caused by different data augmentation, different teacher or training details. $S_1$ (20) / $S_1$ (18) uses ResNet-20 and ResNet-18 as $S_0$ and a NAS-based network as $R_1$.}
\label{table.r3q1}
\begin{tabular}{lcc}
    \toprule
%\checkmark
Architecture  & Acc.~(\%)\\
\midrule
ResNet20 [51]& 70.67\\
ResNet20 [52] & 70.66\\
ResNet20 [53]  & 70.80\\
ResNet20 (ours) & 70.09\\
$S_1$ (20)  & 74.06\\
\midrule
ResNet18 [50]   & 76.87\\
ResNet18 (ours)   & 78.67\\
$S_1$ (18)   & 82.67\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


% \begin{table*}[tb]
%     \begin{center}
%     \caption{Different results on CIFAR-100. For ResNet-110 / ResNet-20, * means taking the 15-degree random rotation into account as \cite{yuan2020revisiting}. The ResNet20* is taught by ResNet110*. 
%     $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is MobileNetv2 / ShuffleNetv2 when $
%     ResNet110 \cite{walawalkar2020online}& - & & 72.64 &  1.73 &  255\\
%     ResNet110*& -&  & 73.23 & 1.73 &  255   \\
%     \midrule
%     \emph{Students}  & & & & \\
%     ResNet20& ResNet110& & 70.09 & 0.28 &  41  \\
%     ResNet20*& ResNet110*& & 70.88 &  0.28 &  41     \\
%     ResNet20* \cite{peng2019correlation}& ResNet110*& & 70.80 &  0.28 &  41 \\
%     ResNet18& ResNet50 & & 78.67 &  11.22 & 557  \\
%     MobileNetv2& ResNet50 & & 75.31 &  2.37 &  68   \\
%     MobileNetv2\cite{yuan2020revisiting}& ResNet50&  & 71.04 & 2.37 &  68  \\
%     ShuffleNetv2& ResNet50&  & 75.92 &   1.36 &  46 \\
%     ShuffleNetv2\cite{yuan2020revisiting}& ResNet50 & & 72.15 &   1.36 &  46  \\
%     \midrule
%     \emph{ResKD students} & & & & &\\
%     $S_1$ (18-L) & ResNet50 & & 82.67 & 16.04 & 1307    \\
%     $S_1$ (18-L)& ResNet50 & $\checkmark$ & 82.37 & 16.04 & 785  \\
%     $S_1$ (18-S) & ResNet50 &  & 80.05 &  11.58 & 620    \\
%     $S_1$ (18-S)& ResNet50 & $\checkmark$ & 80.08 & 11.58 & 576 \\
%     $S_1$ (Mobile)& ResNet50 & & 78.67 & 3.13 & 197 \\
%     $S_1$ (Mobile)& ResNet50 & $\checkmark$ & 78.30 & 3.13  & 101 \\
%     $S_1$ (Shuffle)& ResNet50 &  & 78.64 & 1.72 & 109 \\
%     $S_1$ (Shuffle)& ResNet50 & $\checkmark$ & 78.57 & 1.72  & 65 \\
%     \bottomrule
%     \end{tabular}
    
%     \end{center}
%     \end{table*}
    
    
% \begin{table*}
%     \centering
%     \caption{Experimental results on A, B, and C databases in terms of average MAE.}
%     \begin{tabular}{|c |c |c |c |c | c | c | c | c | c | c| c| c| c|}
%     \hline {Dataset} & {\diagbox{$\alpha$}{$\sigma_s$}} &{1} & {3} & {5} & {7} & {10} \\
%     \hline
     
%     \multirow{5}{*}{A} 
%     & {40} & {0.1703} & {0.1406} & {0.1447} & {0.1078} & {0.0585}   \\
%     \cline{2-7}
%     & {50} & {0.5006} & {0.5360} & {0.3602} & {0.5401} & {0.7303} \\
%     \cline{2-7}
%     & {60} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {70} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {80} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \hline
     
%     \multirow{5}{*}{B} 
%     & {40} & {0.1484} & {0.1406} & {0.1447} & {0.1078} & {0.0585}   \\
%     \cline{2-7}
%     & {50} & {0.5006} & {0.5360} & {0.3602} & {0.5401} & {0.7303} \\
%     \cline{2-7}
%     & {60} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {70} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {80} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \hline
     
%     \multirow{5}{*}{C} 
%     & {40} & {0.1484} & {0.1406} & {0.1447} & {0.1078} & {0.0585}   \\
%     \cline{2-7}
%     & {50} & {0.5006} & {0.5360} & {0.3602} & {0.5401} & {0.7303} \\
%     \cline{2-7}
%     & {60} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {70} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \cline{2-7}
%     & {80} & {0.7367} & {0.7494} & {0.8113} &{0.8429} &{0.9011} \\
%     \hline
     
%     \hline \end{tabular}
%     \label{tab}
%     \end{table*}


% \begin{tabular}{|c|c|c|c|c|}
%     \toprule
% %\checkmark
% Teacher& $S_0$ baseline & $S_0$ (MFLOPs) &  $S_1$ (MFLOPs)&ACC. compared with $S_0$ \\
% ACC. (\%) & ACC.(\%) &ACC. (\%)  &  ACC. (\%)  & ACC. compared with $T$   \\
% MFLOPs & MFLOPs &MFLOPs  &  MFLOPs  & FLOP Percentage of $T$ \\
% \midrule
% %\emph{Baseline}  &  & & & &\\
% & ResNet-18& ResNet-18  & $S_1-18$   &  +1.41\% \\
% &76.80 (75.87\cite{yuan2020revisiting}) &78.67 & 80.08& \textbf{+1.87} (\textbf{+1.92}\cite{yuan2020revisiting})\textbf{\%} \\
% &557 &557& 576& 44.1\%\\
% \cline{2-5}
% ResNet50&MobileNetv2& MobileNetv2& $S_1-Mobile$& \textbf{+2.99} (\textbf{+7.26}\cite{yuan2020revisiting})\textbf{\%}\\
% 78.21(78.16\cite{yuan2020revisiting})&69.30 (68.38 \cite{yuan2020revisiting})& 75.31 (71.04\cite{yuan2020revisiting})& 78.30  & +0.09 (+0.14\cite{yuan2020revisiting})\% \\
% 1306&68& 68& 101 & 7.7\% \\
% \cline{2-5}
% &ShuffleNetv2 & ShuffleNetv2 & $S_1-Shuffle$& +2.65 (+6.42\cite{yuan2020revisiting})\\
% &71.52 (70.34\cite{yuan2020revisiting})& 75.92 (72.15\cite{yuan2020revisiting}) & 78.57 & +0.36 (+0.41\cite{yuan2020revisiting}) \\
% &46& 46& 65& \textbf{5.0\%}\\
% \bottomrule
% \end{tabular}

==> rebuttal_sup/SOTA.tex <==
\begin{table*}[h]
\begin{center}
\caption{
ResKD combined with Normal KD and De-KD [44] for ResNet-18 on CIFAR-100 for different accuracy-cost balance. Teacher network is ResNet-50 when $S_0$ is ResNet-18 and $R_1$ is searched by NAS. 
(big) and (small) means we set our NAS to find a relatively big / small scale $R_1$. 
$S_0$ with (ours) is the results we implemented and $S_1$ is based on this $S_0$.
pt-Res50 is the poor trained ResNet-50 in De-KD.  \textbf{Bold}: The best results out of students.}
\label{SOTA}
\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & KD method & Acc.~(\%) & Acc. gap to $S_0$ (ours / reported)& MFLOPs & additional FLOPs to $S_0$\\
\midrule
ResNet50& - & 78.21  &- & 1306  &-\\
ResNet18& - & 76.80 & - & 557 &-  \\
ResNet18 (ours)& normal & 78.67 &  -& 557 &- \\
ResNet18 [50]& normal & 76.87 &  -& 557 &- \\
$S_1$ (big)& normal & 82.37 &+3.70 / +5.50 & 785 & +228\\
$S_1$ (small)& normal & 80.08 &+1.41 / +3.21& 576& \textbf{+19}\\
\midrule
pt-Res50& - & 46.92  &- & 1306  &-\\
ResNet18 & - & 76.80 & - & 557 &-  \\
ResNet18 (ours)& De-KD & 76.80 &  -& 557 &- \\
ResNet18 [44]& De-KD & 75.87 &  -& 557 &- \\
$S_1$ (big)& De-KD & 81.74 & \textbf{+4.94 / +5.87} & 788 & +231\\
$S_1$ (small)& De-KD & 78.91 &+2.11 / +3.04 & 576 & \textbf{+19}\\
\bottomrule

\end{tabular}
\end{center}
\end{table*}

%\multirow{2}{*}{CIFAR-10}}

% \resizebox{1\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
%     \toprule
% %\checkmark
% $S_0$ baseline& $T$ & $S_0$ (MFLOPs) &  $S_1$ (MFLOPs)&ACC. and extra FLOPs  \\
% ACC. (\%) / MFLOPs & ACC.(\%) / MFLOPs &ACC. (\%) / MFLOPs  &  ACC. (\%) / MFLOPs  & compared with $S_0$  \\
% \midrule
% %\emph{Baseline}  &  & & & &\\
% & normal KD &  & Big $R_1$: 82.37 / 785   &  +3.70\% / 228 (+40.9\% $S_0$) \\
% &78.21(78.16\cite{yuan2020revisiting}) / 1306&78.67 / 557 &small $R_1$: 80.08 / 576& +1.41\%  / \textbf{19 (+3.4\% $S_0$)} \\

% \cline{2-5}
% 76.80 (75.87\cite{yuan2020revisiting}) / 557&De-KD&  & Big $R_1$: 81.74 / 788  &  \textbf{+4.20 (+4.51\cite{yuan2020revisiting})\%} / 231 (41.5\% $S_0$) \\
% & 46.92(45.82\cite{yuan2020revisiting}) / 1306 &77.54(77.23\cite{yuan2020revisiting}) / 557 & small $R_1$: 78.91 / 576& +1.37 (+1.68\cite{yuan2020revisiting})\% / \textbf{19 (+3.4\% $S_0$)} \\

% \bottomrule
% \end{tabular}
% }




% \begin{table*}[tb]
%     \begin{center}
%     \caption{
%     ResKD combined with Normal KD and De-KD \cite{yuan2020revisiting} for ResNet-18 on CIFAR-100 for different accuracy-cost balance. Teacher network is ResNet-50 when $S_0$ is ResNet-18 and $RS_1$ is decided by NAS. pt-Res50 is the poor trained ResNet-50 in De-KD.}
%     \label{SOTA}
    
%     \begin{tabular}{lccccc}
%         \toprule
%     %\checkmark
%     Architecture & Optimizer & SA & Acc.~(\%) & \#Params (M) & MFLOPs\\
%     \midrule
%     \emph{Teacher}  & & & & &\\
%     pt-Res50 & SGD & -  & 46.92 & 23.71 & 1306 \\
%     pt-Res50\cite{yuan2020revisiting} & SGD & - & 45.82 & 23.71 & 1306  \\
%     \midrule
%     \emph{Students}  & & & & &\\
%     $S_0$ & De-KD & - & 77.54 & 11.22 & 557 \\
%     $S_0$\cite{yuan2020revisiting} & De-KD & - & 77.23 & 11.22 & 557 \\
%     \midrule
%     \emph{ResKD students}  & & & & &\\
    
%     $S_1$ (large)  & De-KD&  & 82.13 & 16.04 & 1307 \\
%     $S_1$ (large) &  De-KD & $\checkmark$ & 81.74 & 16.04  & 788 \\
%     $S_1$ (small)  & De-KD&  & 78.89 & 11.58 & 620 \\
%     $S_1$ (small) &  De-KD & $\checkmark$ & 78.91 &  11.58 & 576 \\
    
%     \bottomrule
%     \end{tabular}
    
%     \end{center}
%     \end{table*}
    






==> rebuttal_sup/SOTAimage.tex <==
\begin{table*}[h]
\begin{center}
\caption{
ResKD using different res-students and epochs on ImageNet. The teacher network is ResNet-50 when $S_0$ is ResNet-18 and $R_1$ is searched by NAS. 
$S_0$ with (ours) is the results we implemented and $S_1$ is based on this $S_0$.
%$S_1$ (former) means the result in the first manuscript. 
%(small) means the same architecture as $S_1$ (former).
(small) / (big) means we set our NAS to find a relatively small / big scale $R_1$ with our latest training strategy. 
%(small) and (big) use the step learning rate strategy and 100 epochs.  
\textbf{Bold}: The best results out of students.}
\label{table.SOTAimage}
\begin{tabular}{lccccc}
    \toprule
%\checkmark


\multirow{2}{*}{Architecture}& \multirow{2}{*}{Acc.~(\%)} & Acc. gap to $S_0$& \multirow{2}{*}{\#Params (M)} & \multirow{2}{*}{MFLOPs} & additional\\
 & & (ours / reported) & & & FLOPs to $S_0$\\


%Architecture & Acc.~(\%) & Acc. gap to $S_0$ (ours / reported) & \#Params (M)  & MFLOPs & additional FLOPs to $S_0$\\
\midrule
ResNet50& 75.50  &- &25.56& 4119  &-\\
ResNet18 (ours)& 70.02 & - &11.69& 1821 & - \\
ResNet18 [44]& 70.40 & - &11.69& 1821 & - \\

%$S_1$ (former)&  71.37 & +1.35 / +0.97 & 2216 & +395 \\
$S_1$ (small)&  72.57 & +2.55 / + 2.17&17.40 & 2157 & \textbf{+336} \\
$S_1$ (big)&  \textbf{73.70} & \textbf{+3.68 / +3.30}&19.71 & 2342 & +521 \\



%\multirow{3}{*}{CIFAR-10}}&  72.41 & +2.39 / +2.01 & \textbf{2156} & \textbf{+335} \\

\bottomrule

\end{tabular}
\end{center}
\end{table*}


% \resizebox{1\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
%     \toprule
% %\checkmark
% $S_0$ baseline& $T$ & $S_0$ (MFLOPs) &  $S_1$ (MFLOPs)&ACC. and extra FLOPs  \\
% ACC. (\%) / MFLOPs & ACC.(\%) / MFLOPs &ACC. (\%) / MFLOPs  &  ACC. (\%) / MFLOPs  & compared with $S_0$  \\
% \midrule
% %\emph{Baseline}  &  & & & &\\
% & normal KD &  & Big $R_1$: 82.37 / 785   &  +3.70\% / 228 (+40.9\% $S_0$) \\
% &78.21(78.16\cite{yuan2020revisiting}) / 1306&78.67 / 557 &small $R_1$: 80.08 / 576& +1.41\%  / \textbf{19 (+3.4\% $S_0$)} \\

% \cline{2-5}
% 76.80 (75.87\cite{yuan2020revisiting}) / 557&De-KD&  & Big $R_1$: 81.74 / 788  &  \textbf{+4.20 (+4.51\cite{yuan2020revisiting})\%} / 231 (41.5\% $S_0$) \\
% & 46.92(45.82\cite{yuan2020revisiting}) / 1306 &77.54(77.23\cite{yuan2020revisiting}) / 557 & small $R_1$: 78.91 / 576& +1.37 (+1.68\cite{yuan2020revisiting})\% / \textbf{19 (+3.4\% $S_0$)} \\

% \bottomrule
% \end{tabular}
% }




% \begin{table*}[tb]
%     \begin{center}
%     \caption{
%     ResKD combined with Normal KD and De-KD \cite{yuan2020revisiting} for ResNet-18 on CIFAR-100 for different accuracy-cost balance. Teacher network is ResNet-50 when $S_0$ is ResNet-18 and $RS_1$ is decided by NAS. pt-Res50 is the poor trained ResNet-50 in De-KD.}
%     \label{SOTA}
    
%     \begin{tabular}{lccccc}
%         \toprule
%     %\checkmark
%     Architecture & Optimizer & SA & Acc.~(\%) & \#Params (M) & MFLOPs\\
%     \midrule
%     \emph{Teacher}  & & & & &\\
%     pt-Res50 & SGD & -  & 46.92 & 23.71 & 1306 \\
%     pt-Res50\cite{yuan2020revisiting} & SGD & - & 45.82 & 23.71 & 1306  \\
%     \midrule
%     \emph{Students}  & & & & &\\
%     $S_0$ & De-KD & - & 77.54 & 11.22 & 557 \\
%     $S_0$\cite{yuan2020revisiting} & De-KD & - & 77.23 & 11.22 & 557 \\
%     \midrule
%     \emph{ResKD students}  & & & & &\\
    
%     $S_1$ (large)  & De-KD&  & 82.13 & 16.04 & 1307 \\
%     $S_1$ (large) &  De-KD & $\checkmark$ & 81.74 & 16.04  & 788 \\
%     $S_1$ (small)  & De-KD&  & 78.89 & 11.58 & 620 \\
%     $S_1$ (small) &  De-KD & $\checkmark$ & 78.91 &  11.58 & 576 \\
    
%     \bottomrule
%     \end{tabular}
    
%     \end{center}
%     \end{table*}
    






==> rebuttal_sup/one_teacher.tex <==
\begin{table}[h]
    \begin{center}
    \caption{
        Performance on CIFAR-100 with different supervision. $T$ is ResNet-110, $S_0$ is ResNet-20 and $R_{1}$ is ResNet-14. If we only use $T$ or GT to realize residual-guided learning, it will not work.}
    \label{tab:one_teacher}

    \begin{tabular}{lcccc}
        \toprule
    %\checkmark
    Architecture & Supervision & Acc.~(\%) & \#Params (M) & MFLOPs\\
    \midrule
    \emph{Baselines}  &  & & & \\
    $T$ & GT  & 72.44 & 1.734 &  255\\
    $S_0$ & GT &  68.82  & 0.276 &  41\\
    
    \midrule
    \emph{Student}  & & & & \\
    $S_0$ & $T$ and GT & 70.09  & 0.276 &  41 \\
    
    \midrule
    \emph{ResKD students}  & & & &\\
    $S_1$ & $T$ and GT  & 71.96 & 0.276 &  68 \\
    $S_1$ & $T$  &  < 50 & 0.276 &  68\\
    $S_1$ & GT & < 50 & 0.276 &  68 \\
    \bottomrule
    \end{tabular}

    \end{center}
    \end{table}
    
    
    

==> rebuttal_sup/vgg_inceptioncifar.tex <==
\begin{table*}[h]
\begin{center}
\caption{
Performance on CIFAR-10 / CIFAR-100. $R_{1}$ is a res-student whose architecture is searched by NAS. The results of $S_1$ are combined with sample-adaptive inference. $S_1$ (VGG) / $S_1$ (Xception) / $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is VGG11BN / Xception / MobileNetv2 / ShuffleNetv2 and $R_1$ is a NAS-based network. \textbf{Bold}: The best results out of students.
    }
\label{table.vgg_inception_cifar}

\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & Teacher & Acc.~(\%) & Acc. improvement to $S_0$ ~(\%) & MFLOPs & Extra FLOPs to $S_0$\\
\toprule
\textbf{Teachers} \\
Inceptionv3 & -  & 95.28 / 79.40 &- & 3399 / 3400 &-\\
VGG19BN & -  & 93.70 / 71.50 &- &418 / 419&-\\
ResNet50& - & 95.33 / 78.21  &- & 1305 / 1306  &-\\
\toprule
\textbf{Students} \\
%Xception & -  & 94.58 / 78.13&- &1134 / 1134&- \\
Xception & Inceptionv3  & 94.99 / 78.58& - & 1134 / 1134 &- \\
$S_1$ (Xception) & Inceptionv3  & 96.15 / 83.13& +1.16 / +4.55& 1163 / 1394  &+29 / +260\\
\midrule
%VGG11BN & -  & 91.99 / 68.96 & -& 172 / 173&-\\
VGG11BN & VGG19BN  & 92.17 / 71.46 &- &172 / 173 &-  \\
$S_1$ (VGG) & VGG19BN  & 94.01  / 76.58  & \textbf{+1.84} / \textbf{+5.12} &206 / 203 & +34 / +30 \\
\midrule
%MobileNetv2& - & 92.75 / 69.30 & -& 67 / 68 &- \\
MobileNetv2& ResNet50 &93.21 / 75.31& -& 67 / 68 & - \\
$S_1$ (Mobile)& ResNet50 & 93.83 / 78.30 & +0.62 / +2.99 & 70 / 101& \textbf{+3} / +33\\
\midrule
%ShuffleNetv2& - &93.4 / 71.52 &- & 45 / 46 & - \\
ShuffleNetv2& ResNet50 &93.98 / 75.92 & -& 45 / 46 &-\\
$S_1$ (Shuffle)& ResNet50 & 94.56 / 78.57 & +0.58 / +2.65 & 49 / 65 & +4 / \textbf{+19} \\
\bottomrule

\end{tabular}

\end{center}
\end{table*}


% \begin{table*}[h]
%     \begin{center}
%     \caption{
%     Performance on CIFAR-10 / CIFAR-100. $R_{1}$ is a res-student whose architecture is searched by NAS. The results of $S_1$ are combined with sample-adaptive inference. $S_1$ (VGG) / $S_1$ (Xception) / $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is VGG11BN / Xception / MobileNetv2 / ShuffleNetv2 and $R_1$ is a NAS-based network.
%         }
%     \label{vgg_inception_cifar}
    
%     \begin{tabular}{lcccc}
%         \toprule
%     %\checkmark
%     Architecture & Teacher & Acc.~(\%) & \#Params (M) & MFLOPs\\
%     \midrule
%     \emph{Baseline}  &  & & & \\
%     VGG19BN & -  & 93.70 / 71.50 &38.96 / 39.33 &418 / 419\\
%     VGG11BN & -  & 91.99 / 68.96 & 28.15 / 28.52 & 172 / 173\\
%     Inceptionv3 & -  & 95.28 / 79.40 & 22.13 / 22.32 & 3399 / 3400 \\
%     Xception & -  & 94.58 / 78.13 & 20.83 / 21.01 & 1134 / 1134 \\
%     ResNet50& - & 95.33 / 78.21 & 23.52 / 23.71 &  1305 / 1306  \\
%     MobileNetv2& - & 92.75 / 69.30 & 2.25 / 2.37 & 67 / 68  \\
%     ShuffleNetv2& - &93.4 / 71.52 & 1.27 / 1.36 & 45 / 46   \\
%     \midrule
%     \emph{Students}  & & & & \\
%     VGG11BN & VGG19BN  & 92.17 / 71.46 & 28.15 / 28.52 & 172 / 173   \\
%     Xception & Inceptionv3  & 94.99 / 78.58 &  20.83 / 21.01 & 1134 / 1134  \\
%     MobileNetv2& ResNet50 &93.21 / 75.31 & 2.25 / 2.37 & 67 / 68  \\
%     ShuffleNetv2& ResNet50 &93.98 / 75.92 &  1.27 / 1.36 & 45 / 46 \\
    
%     \midrule
%     \emph{ResKD students}  & & & &\\
%     $S_1$ (VGG) & VGG19BN  & 94.01 / 79.46 & 32.90 / 33.27 & 206 / 433  \\
%     $S_1$ (Xception) & Inceptionv3  & 96.15 / 83.13 & 25.58 / 25.76 & 1163 / 1394  \\
%     $S_1$ (Mobile)& ResNet50 & 93.83 / 78.30 & 2.81 / 3.13  & 70 / 101 \\
%     $S_1$ (Shuffle)& ResNet50 & 94.56 / 78.57 & 1.99 / 1.72  & 49 / 65 \\
    
%     \bottomrule
%     \end{tabular}
    
%     \end{center}
%     \end{table*}

==> rebuttal_sup/vgg_inceptionimage.tex <==
\begin{table*}[tb]
\begin{center}
\caption{
aaaaa
    }
\label{vgg_inception_image}

\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & Teacher & Acc.~(\%) & \#Params (M) & MFLOPs& Energy \\
\midrule
\emph{Baseline}  &  & & & &\\
VGG19& -  & 65.41 /  &  &    & \\
VGG11& -  & 61.42 /  &  &    & \\
Inceptionv3& -  &  /  &  &    & \\
Xception& -  &  /  &  &    & \\
\midrule
\emph{Students}  & & & & &\\
VGG11& VGG19  & 62.86 /  &  &    & \\
Xception& Inceptionv3  &  /  &  &    & \\

\midrule
\emph{ResKD students}  & & & & &\\
VGG11$+$RS1& VGG19  & 65.62 / &  &    & \\
Xception$+$RS1& Inceptionv3  &  &  &    & \\


\bottomrule
\end{tabular}

\end{center}
\end{table*}




==> tables/100_other_final.tex <==
\begin{table}[tb]
    \begin{center}
    \caption{
        Performance on CIFAR-100. $R_{1}$ is a res-student whose architecture is searched by NAS. The results of $S_1$ are combined with sample-adaptive inference. $S_1$ (VGG) / $S_1$ ((Xception) / $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is VGG11BN / Xception / MobileNetv2 / ShuffleNetv2 and $R_1$ is a NAS-based network. $S_1$ (18-L) means we use ResNet18 as $S_0$ and a larger NAS-based network $R_1$ to achieve a better performance when $S_1$ (18-L) means we use a smaller NAS-based network $R_1$ to cost less. \textbf{Bold}: The best results out of students. \ul{Underline}: The second best  results out of students.}
        
    \label{tab:100_other}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
    %\checkmark
    Architecture & Teacher & Acc.~(\%) & \#Params (M) & MFLOPs\\
    \midrule
    \emph{Baseline}  &  & & & \\
    VGG19BN & -  & 71.50 & 39.33 &419\\
    VGG11BN & -  &  68.96 &  28.52 & 173\\
    Inceptionv3 & -  &  79.40 &  22.32 & 3400 \\
    Xception & -  & 78.13 &  21.01 &  1134 \\
    ResNet50& - & 78.21 & 23.71 &  1306  \\
    ResNet50\cite{yuan2020revisiting}& - & 78.16 & 23.71 & 1306   \\
    ResNet18& - & 76.80 & 11.22 & 557   \\
    ResNet18\cite{yuan2020revisiting}& - & 75.87 &   11.22 & 557   \\
    MobileNetv2& - & 69.30 & 2.37 &  68  \\
    MobileNetv2\cite{yuan2020revisiting}& - &  68.38  & 2.37 & 68  \\
    ShuffleNetv2& - & 71.52 &  1.36 & 46   \\
    ShuffleNetv2\cite{yuan2020revisiting}& - & 70.34  & 1.36 &  46   \\
    
    \midrule
    \emph{Students}  & & & & \\
    VGG11BN & VGG19BN  &  71.46 & 28.52 & 173   \\
    Xception & Inceptionv3  &  78.58 &   21.01 &  1134  \\
    ResNet18& ResNet50 & 78.67 &  11.22 & 557  \\
    MobileNetv2& ResNet50 &75.31 & 2.37 &  68  \\
    MobileNetv2\cite{yuan2020revisiting}& ResNet50&  71.04 & 2.37 & 68  \\
    ShuffleNetv2& ResNet50 &75.92 &  \textbf{1.36} & \textbf{46} \\
    ShuffleNetv2\cite{yuan2020revisiting}& ResNet50 & 72.15 &  \textbf{1.36} &  \textbf{46}  \\
    
    \midrule
    \emph{ResKD students}  & & & &\\
    $S_1$ (VGG) & VGG19BN  & 79.46 & 33.27 & 433  \\
    $S_1$ (Xception) & Inceptionv3  & \textbf{83.13} & 25.76 & 1394  \\
    $S_1$ (18-L)& ResNet50 & \ul{82.37} & 16.04 & 785  \\
    $S_1$ (18-S)& ResNet50 & 80.08 & 11.58 & 620 \\
    $S_1$ (Mobile)& ResNet50 &  78.30 & 3.13  & 101 \\
    $S_1$ (Shuffle)& ResNet50 &  78.57 &  \ul{1.72}  &  \ul{65} \\
    
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \end{table}
    
    
    

==> tables/10_100_other_final.tex <==
\begin{table}[tb]
\begin{center}
\caption{
Performance on CIFAR-10 / CIFAR-100. $R_{1}$ is a res-student whose architecture is searched by NAS. $S_1$ means using both $S_0$ and $R_1$. \textbf{Bold}: The best results out of students. \ul{Underline}: The second best  results out of students.
    }
\label{tab:vgg_inception_cifar}
\resizebox{0.55\textwidth}{!}{
\begin{tabular}{lcccc}
    \toprule
%\checkmark
Architecture & Teacher & Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Baseline}  &  & & & \\
VGG19BN & -  & 93.70 / 71.50 &38.96 / 39.33 &418 / 419\\
VGG11BN & -  & 92.23 / 68.96 & 28.15 / 28.52 & 172 / 173\\
Inceptionv3& -  & 95.28 / 79.40 & 22.13 / 22.32 & 3403 / 3404 \\
Xception& -  & 94.58 / 78.13 & 20.83 / 21.01 & 2266 / 2267 \\
\midrule
\emph{Students}  & & & & \\
VGG11BN & VGG19BN  &  / 71.46 & 28.15 / 28.52 & 172 / 173   \\
Xception& Inceptionv3  & 95.03 / 78.58 &  20.83 / 21.01 & 2266 / 2267  \\

\midrule
\emph{ResKD students}  & & & &\\
VGG11BN$+R_1$ & VGG19BN  &  / 80.53 &  &   \\
Xception$+R_1$ & Inceptionv3  & 96.15 / 83.13 &  &   \\


\bottomrule
\end{tabular}
}
\end{center}
\end{table}



==> tables/10_other_final.tex <==
\begin{table}[h]
    \begin{center}
    \caption{
        Performance on CIFAR-10 / CIFAR-100. $R_{1}$ is a res-student whose architecture is searched by NAS. The results of $S_1$ are combined with sample-adaptive inference. $S_1$ (VGG) / $S_1$ ((Xception) / $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is VGG11BN / Xception / MobileNetv2 / ShuffleNetv2 and $R_1$ is a NAS-based network. \textbf{Bold}: The best results out of students. \ul{Underline}: The second best  results out of students.}
    \label{tab:10_other}
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
    %\checkmark
    Architecture & Teacher & Acc.~(\%) & \#Params (M) & MFLOPs\\
    \midrule
    \emph{Baseline}  &  & & & \\
    VGG19BN & -  & 93.70 &38.96  &418 \\
    VGG11BN & -  & 91.99  & 28.15 & 172\\
    Inceptionv3 & -  & 95.28  & 22.13 & 3399\\
    Xception & -  & 94.58  & 20.83 & 1134 \\
    ResNet50& - & 95.33  & 23.52  &  1305  \\
    MobileNetv2& - & 92.75 & 2.25  & 67  \\
    ShuffleNetv2& - &93.4  & 1.27  & 45   \\

    
    \midrule
    \emph{Students}  & & & & \\
    VGG11BN & VGG19BN  & 92.17& 28.15 & 172 \\
    Xception & Inceptionv3  & \ul{94.99} &  20.83& 1134  \\
    MobileNetv2& ResNet50 &93.21  & 2.25 & 67 \\
    ShuffleNetv2& ResNet50 &93.98  &  \textbf{1.27}  & \textbf{45} \\
 
    
    \midrule
    \emph{ResKD students}  & & & &\\
    $S_1$ (VGG) & VGG19BN  & 94.01 & 32.90 & 206 \\
    $S_1$ (Xception) & Inceptionv3  & \textbf{96.15}  & 25.58 & 1163 \\
    $S_1$ (Mobile)& ResNet50 & 93.83  & 2.81  & 70 \\
    $S_1$ (Shuffle)& ResNet50 & 94.56 & \ul{1.99}  & \ul{49}  \\
    
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \end{table}
    
    
    

==> tables/morecifar_main.tex <==
\begin{table}[h]
\begin{center}
\caption{
\ul{Performance on CIFAR-10 / CIFAR-100. $R_{1}$ is a res-student whose architecture is searched by NAS. The results of ResKD students are combined with sample-adaptive inference. $S_1$ (VGG) / $S_1$ ((Xception) / $S_1$ (Mobile) / $S_1$ (Shuffle) means $S_0$ is VGG11BN / Xception / MobileNetv2 / ShuffleNetv2 and $R_1$ is a NAS-based network.}
    }
\label{vgg_inception_cifar}

\begin{tabular}{lcccc}
    \toprule
%\checkmark
Architecture & Teacher & Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Baseline}  &  & & & \\
VGG19BN & -  & 93.70 / 71.50 &38.96 / 39.33 &418 / 419\\
VGG11BN & -  & 91.99 / 68.96 & 28.15 / 28.52 & 172 / 173\\
Inceptionv3 & -  & 95.28 / 79.40 & 22.13 / 22.32 & 3399 / 3400 \\
Xception & -  & 94.58 / 78.13 & 20.83 / 21.01 & 1134 / 1134 \\
ResNet50& - & 95.33 / 78.21 & 23.52 / 23.71 &  1305 / 1306  \\
MobileNetv2& - & 92.75 / 69.30 & 2.25 / 2.37 & 67 / 68  \\
ShuffleNetv2& - &93.4 / 71.52 & 1.27 / 1.36 & 45 / 46   \\
ResNet50\cite{yuan2020revisiting}& - & - / 78.16 & - / 23.71 & - / 1306   \\
MobileNetv2\cite{yuan2020revisiting}& - & - / 68.38  & - / 2.37 & - / 68  \\
ShuffleNetv2\cite{yuan2020revisiting}& - & - / 70.34  &   - / 1.36 &  - / 46   \\

\midrule
\emph{Students}  & & & & \\
VGG11BN & VGG19BN  & 92.17 / 71.46 & 28.15 / 28.52 & 172 / 173   \\
Xception & Inceptionv3  & 94.99 / 78.58 &  20.83 / 21.01 & 1134 / 1134  \\
MobileNetv2& ResNet50 &93.21 / 75.31 & 2.25 / 2.37 & 67 / 68  \\
ShuffleNetv2& ResNet50 &93.98 / 75.92 &  1.27 / 1.36 & 45 / 46 \\
MobileNetv2\cite{yuan2020revisiting}& ResNet50&  - / 71.04 & - / 2.37 & - / 68  \\
ShuffleNetv2\cite{yuan2020revisiting}& ResNet50 & - / 72.15 &   - / 1.36 &  - / 46  \\

\midrule
\emph{ResKD students}  & & & &\\
$S_1$ (VGG) & VGG19BN  & 94.01 / 79.46 & 32.90 / 33.27 & 206 / 433  \\
$S_1$ (Xception) & Inceptionv3  & 96.15 / 83.13 & 25.58 / 25.76 & 1163 / 1394  \\
$S_1$ (Mobile)& ResNet50 &  / 78.30 & / 3.13  & / 101 \\
$S_1$ (Shuffle)& ResNet50 &  / 78.57 &  / 1.72  &  / 65 \\

\bottomrule
\end{tabular}

\end{center}
\end{table}




==> tables/res_100_all.tex <==
\begin{table}[h]
\begin{center}
\caption{
    Effect of sample-adaptive inference and KD methods on CIFAR-10/100. $T$ is ResNet-110, $S_0$ is ResNet-20, and $R_1$ is ResNet-14. $S_1$ means using both $S_0$ and $R_1$. 
    %NAS14 denotes a network searched by NAS with comparable parameters to ResNet-14.
    Using sample-adaptive inference, the performance would edge down but the computational cost would be saved considerably. Our ResKD framework can be applied to different KD methods.  \textbf{Bold}: The best results out of students. \ul{Underline}: The second best results out of students.}

%
\label{tab:res_100_all}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
    \toprule
%\checkmark
Architecture & Optimizer & SA & Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Teacher}  & & & & &\\
Res110 & SGD &  & 94.19 / 72.44 & 1.728 / 1.734 &  255 / 255\\
\midrule
\emph{Students}  & & & & &\\
%$S_0$ & SGD &  & 91.80 / 68.82 & 0.276 &  41\\
Res20 & KD &  & 93.06 / 70.09  & 0.270 / 0.276 &  \textbf{41} / \textbf{41}\\
Res20 & DML &  & 92.53 / 68.96 & 0.270 / 0.276 &  \textbf{41} / \textbf{41}\\
Res20 & RKD &  & 92.45 / 68.88 & 0.270 / 0.276 &  \textbf{41} / \textbf{41}\\
Res20 & FitNets &   & 92.88 / 68.53 & 0.270 / 0.276 &  \textbf{41} / \textbf{41}\\
\midrule
\emph{ResKD students}  & & & & &\\
Res20-14 & KD &  & 93.27 / \textbf{71.96} & 0.442 /  0.454 &  68 / 68\\
Res20-14 & KD & $\checkmark$ & 93.27 / \ul{71.94} &  0.442 / 0.454 &  \ul{44} / \ul{52}\\

% Res20-NAS14 & KD &  & \textbf{93.92} / \textbf{74.06} & 0.453 /  0.485 &  79 / 81\\
% Res20-NAS14 & KD & $\checkmark$ & \textbf{93.92} / \textbf{74.06} &  0.453 / 0.485 &  46 / 59\\

Res20-14 & DML &   & 92.88 / 70.30 & 0.442 /  0.454 &  68 / 68\\
Res20-14 & DML &  $\checkmark$ & 92.88 / 70.29 & 0.442 /   0.454 &  50 / 58\\

Res20-14 & RKD &   & 93.17 / 71.52 & 0.442 /  0.454 &  68 / 68\\
Res20-14 & RKD &  $\checkmark$ & 93.17 / 71.52 & 0.442 /  0.454 &  48 / 55\\

Res20-14 & FitNets &   & \textbf{93.65} / 71.22 & 0.442 /  0.454 &  68 / 68\\
Res20-14 & FitNets &  $\checkmark$ & \ul{93.63} / 71.21  & 0.442 /  0.454 &  \ul{44} / 55\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

%\begin{table}[tb]
%    \begin{center}
%    \caption{Performance of ResNet series networks  on CIFAR-100 using different different KD methods and with/without sample-adaptive inference. The teacher network is ResNet-110. $S_0$ is ResNet-20 and $R_1$ is ResNet-14. $S_1$ means using both $S_0$ and $R_1$. }
%    \label{tab:res_100_all}
%    \resizebox{0.48\textwidth}{!}{
%    \begin{tabular}{lccccc}
%        \toprule
%    Architecture & Optimizer & SA & Acc.~(\%) & \#Params (M) & MFLOPs\\
%    \midrule
%    \emph{Teacher}  & & & & &\\
%    Res110 & SGD &  & 72.44 & 1.734 &  255\\
%    \midrule
%    \emph{Students}  & & & & &\\
%    $S_0$ & SGD &  & 68.82 & 0.276 &  41\\
%    $S_0$ & KD &  & 70.09 & 0.276 &  41\\
%    $S_0$ & DML &  & 68.29 & 0.276 &  41\\
%    \midrule
%    \emph{ResKD students}  & & & & &\\
%    $S_1$ & KD &  & 71.96 &  0.454 &  68\\
%    $S_1$ & KD & $\checkmark$ & \textbf{71.94} &  0.454 &  \textbf{52}\\
%    $S_1$ & DML &   & 70.05 & 0.454 &  68\\
%    $S_1$ & DML &  $\checkmark$ & \textbf{70.01} &  0.454 &  \textbf{52}\\
%    \bottomrule
%    \end{tabular}
%    }
%    \end{center}
%    \end{table}

==> tables/t-imagenet.tex <==
\begin{table*}[tb]
\begin{center}
\caption{Performance on Tiny-ImageNet / ImageNet. $T$ is ResNet-50, $S_0$ is a ResNet-18, $R_{1}$ is a res-student whose architecture is searched by NAS. $S_1$ means using both $S_0$ and $R_1$. `SA' means using our sample-adaptive strategy at inference time. } 
\label{tab:t-Imagenet}
\begin{tabular}{lcccc}
\toprule
Architecture & SA  & Acc.~(\%) & \#Params (M) & MFLOPs\\
\midrule
\emph{Teacher}  & & &\\
Res50 &  & 70.42 / 75.50 & 23.92 / 25.56 & 4117 / 4119\\
\midrule
\emph{Students}  & & &\\
$S_0$ &  & 67.90 / 70.02 & 11.28 / 11.69 & 1821 / 1821\\
\midrule
\emph{ResKD students}  & & &\\
$S_{1}$ &  & 68.98 / 71.37 & 16.38 / 17.40 & 2453 / 2454\\
$S_{1}$ & $\checkmark$ &  \textbf{68.99} / \textbf{71.37} & 16.38 / 17.40 &  \textbf{2206} /  \textbf{2216}\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

%\begin{table}[tb]
%    \begin{center}
%    \caption{Performance on Tiny-ImageNet / ImageNet. $T$ is ResNet-50, $S_0$ is a ResNet-18, $R_{1}$ is a res-student whose architecture is searched by NAS. $S_1$ means using both $S_0$ and $R_1$. `SA' means using our sample-adaptive strategy at inference time. } 
%    \label{tab:t-Imagenet}
%    \begin{tabular}{lccc}
%    \toprule
%    Architecture & Acc.~(\%) & \#Params (M) & MFLOPs\\
%    \midrule
%    \emph{Teacher}  & & &\\
%    Res50 & 70.42 / 75.50 & 23.92 / 25.56 & 4117 / 4119\\
%    \midrule
%    \emph{Students}  & & &\\
%    $S_0$ (SGD) & 66.32 / 69.16 & 11.28 / 11.69 & 1821 / 1821\\
%    $S_0$ (KD) & 67.90 / 70.02 & 11.28 / 11.69 & 1821 / 1821\\
%    \midrule
%    \emph{ResKD students}  & & &\\
%    $S_{1}$ & 68.98 / 71.37 & 16.38 / 17.40 & 2453 / 2454\\
%    $S_{1}$ (SA) &  \textbf{68.99} / \textbf{71.37} & 16.38 / 17.40 &  \textbf{2206} /  \textbf{2216}\\
%    \bottomrule
%    \end{tabular}
%    \end{center}
%    \end{table}
